Chemical signatures of planets: beyond solar-twins

Elemental abundance studies of solar twin stars suggest that the solar chemical composition contains signatures of the formation of terrestrial planets in the solar system, namely small but significant depletions of the refractory elements. To test this hypothesis, we study stars which, compared to solar twins, have less massive convective envelopes (therefore increasing the amplitude of the predicted effect) or are, arguably, more likely to host planets (thus increasing the frequency of signature detections). We measure relative atmospheric parameters and elemental abundances of a late-F type dwarf sample (52 stars) and a sample of metal-rich solar analogs (59 stars). We detect refractory-element depletions with amplitudes up to about 0.15 dex. The distribution of depletion amplitudes for stars known to host gas giant planets is not different from that of the rest of stars. The maximum amplitude of depletion increases with effective temperature from 5650 K to 5950 K, while it appears to be constant for warmer stars (up to 6300 K). The depletions observed in solar twin stars have a maximum amplitude that is very similar to that seen here for both of our samples. Gas giant planet formation alone cannot explain the observed distributions of refractory-element depletions, leaving the formation of rocky material as a more likely explanation of our observations. More rocky material is necessary to explain the data of solar twins than metal-rich stars, and less for warm stars. However, the sizes of the stars' convective envelopes at the time of planet formation could be regulating these amplitudes. Our results could be explained if disk lifetimes were shorter in more massive stars, as independent observations indeed seem to suggest.

==> abundances.tex <==
HIP & $\Delta$[C/H]  & $\sigma$ & $\Delta$[O/H]  & $\sigma$ & $\Delta$[Na/H] & $\sigma$ & $\Delta$[Mg/H] & $\sigma$ & $\Delta$[Al/H] & $\sigma$ & $\Delta$[Si/H] & $\sigma$ & $\Delta$[S/H]  & $\sigma$ & $\Delta$[Ca/H] & $\sigma$ & $\Delta$[Sc/H] & $\sigma$ & $\Delta$[Ti/H] & $\sigma$ & $\Delta$[V/H]  & $\sigma$ & $\Delta$[Cr/H] & $\sigma$ & $\Delta$[Mn/H] & $\sigma$ & $\Delta$[Co/H] & $\sigma$ & $\Delta$[Ni/H] & $\sigma$ & $\Delta$[Cu/H] & $\sigma$ & $\Delta$[Zn/H] & $\sigma$ & $\Delta$[Ba/H] & $\sigma$ \\ \hline
\\ \multicolumn{37}{c}{wm: late F-dwarfs} \\ \hline
   522 & -0.059 & 0.036 & -0.066 & 0.011 & -0.183 & 0.011 & -0.125 & 0.050 & -0.091 & 0.033 & -0.066 & 0.040 & -0.024 & 0.042 & -0.069 & 0.034 & -0.121 & 0.011 & -0.067 & 0.083 & -0.082 & 0.069 & -0.067 & 0.041 & -0.138 & 0.039 & -0.131 & 0.021 & -0.134 & 0.050 & -0.153 & 0.081 & -0.076 & 0.050 & -0.016 & 0.028 \\
  3119 & -0.106 & 0.033 & -0.031 & 0.002 & -0.192 & 0.011 & -0.074 & 0.050 & -0.150 & 0.016 & -0.100 & 0.027 & -0.143 & 0.061 & -0.071 & 0.029 & -0.128 & 0.024 & -0.057 & 0.048 & -0.090 & 0.092 & -0.082 & 0.019 & -0.087 & 0.071 & -0.108 & 0.052 & -0.122 & 0.043 & -0.174 & 0.001 & -0.088 & 0.050 &  0.034 & 0.017 \\
  3236 & -0.213 & 0.044 & -0.117 & 0.003 & -0.242 & 0.003 & -0.085 & 0.050 & -0.217 & 0.046 & -0.163 & 0.022 & -0.205 & 0.042 & -0.082 & 0.052 & -0.161 & 0.015 & -0.069 & 0.061 & -0.088 & 0.069 & -0.089 & 0.062 & -0.159 & 0.083 & -0.105 & 0.125 & -0.193 & 0.048 & -0.270 & 0.031 & -0.196 & 0.050 &  0.072 & 0.007 \\
  3540 & -0.146 & 0.080 & -0.164 & 0.005 & -0.288 & 0.003 & -0.121 & 0.050 & -0.243 & 0.042 & -0.202 & 0.019 & -0.173 & 0.065 & -0.164 & 0.051 & -0.254 & 0.033 & -0.202 & 0.087 & -0.241 & 0.118 & -0.205 & 0.049 & -0.247 & 0.064 & -0.163 & 0.091 & -0.256 & 0.059 & -0.338 & 0.034 & -0.136 & 0.050 & -0.121 & 0.068 \\
  5862 & -0.041 & 0.011 & -0.032 & 0.005 & -0.097 & 0.004 & -0.049 & 0.050 & -0.073 & 0.047 & -0.049 & 0.015 & -0.041 & 0.051 & -0.032 & 0.033 & -0.057 & 0.022 & -0.045 & 0.029 & -0.064 & 0.040 & -0.037 & 0.054 & -0.025 & 0.051 & -0.026 & 0.070 & -0.048 & 0.044 & -0.058 & 0.006 & -0.049 & 0.050 & -0.025 & 0.060 \\
  5985 & -0.157 & 0.060 & -0.136 & 0.005 & -0.228 & 0.008 & -0.106 & 0.050 & -0.202 & 0.022 & -0.164 & 0.029 & -0.169 & 0.062 & -0.124 & 0.032 & -0.168 & 0.033 & -0.119 & 0.057 & -0.142 & 0.066 & -0.122 & 0.040 & -0.165 & 0.052 & -0.164 & 0.076 & -0.169 & 0.035 & -0.182 & 0.051 & -0.167 & 0.050 & -0.087 & 0.040 \\
  7978 & -0.260 & 0.076 & -0.230 & 0.020 & -0.440 & 0.008 & -0.201 & 0.050 & -0.335 & 0.064 & -0.286 & 0.028 & -0.261 & 0.084 & -0.205 & 0.058 & -0.294 & 0.048 & -0.189 & 0.071 & -0.284 & 0.050 & -0.244 & 0.040 & -0.309 & 0.045 & -0.267 & 0.071 & -0.327 & 0.040 & -0.354 & 0.058 & -0.296 & 0.050 & -0.045 & 0.035 \\
  8548 & -0.089 & 0.059 & -0.142 & 0.006 & -0.236 & 0.026 & -0.110 & 0.050 & -0.206 & 0.031 & -0.197 & 0.016 & -0.168 & 0.083 & -0.199 & 0.037 & -0.194 & 0.012 & -0.196 & 0.050 & -0.218 & 0.073 & -0.201 & 0.046 & -0.178 & 0.059 & -0.183 & 0.083 & -0.210 & 0.037 & -0.212 & 0.034 & -0.165 & 0.050 & -0.204 & 0.034 \\
 12653 & -0.106 & 0.036 & -0.032 & 0.012 & -0.179 & 0.030 & -0.171 & 0.050 & -0.117 & 0.056 & -0.092 & 0.019 & -0.113 & 0.055 & -0.043 & 0.035 & -0.122 & 0.018 & -0.032 & 0.063 & -0.063 & 0.071 & -0.029 & 0.044 & -0.081 & 0.004 & -0.097 & 0.100 & -0.101 & 0.042 & -0.171 & 0.057 & -0.108 & 0.050 &  0.074 & 0.031 \\
 12764 & -0.076 & 0.041 & -0.069 & 0.010 & -0.229 & 0.011 & -0.072 & 0.050 & -0.182 & 0.028 & -0.131 & 0.019 & -0.121 & 0.033 & -0.122 & 0.018 & -0.132 & 0.024 & -0.097 & 0.083 & -0.118 & 0.084 & -0.128 & 0.043 & -0.182 & 0.035 & -0.137 & 0.043 & -0.160 & 0.041 & -0.211 & 0.005 & -0.114 & 0.050 & -0.093 & 0.005 \\
 14194 & -0.142 & 0.033 & -0.022 & 0.010 & -0.167 & 0.013 & -0.143 & 0.050 & -0.113 & 0.042 & -0.061 & 0.022 & -0.194 & 0.130 & -0.013 & 0.044 & -0.089 & 0.019 &  0.015 & 0.075 &  0.019 & 0.090 & -0.013 & 0.037 & -0.032 & 0.053 &  0.000 & 0.073 & -0.065 & 0.052 & -0.168 & 0.035 & -0.110 & 0.050 &  0.085 & 0.035 \\
 14857 & -0.102 & 0.071 & -0.091 & 0.010 & -0.204 & 0.016 & -0.043 & 0.050 & -0.110 & 0.038 & -0.103 & 0.017 & -0.141 & 0.022 & -0.069 & 0.036 & -0.105 & 0.023 & -0.080 & 0.069 & -0.107 & 0.041 & -0.073 & 0.025 & -0.111 & 0.043 & -0.069 & 0.075 & -0.120 & 0.037 & -0.199 & 0.008 & -0.110 & 0.050 & -0.029 & 0.024 \\
 14954 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.050 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.050 &  0.000 & 0.000 \\
 17819 & -0.000 & 0.056 & -0.050 & 0.013 & -0.065 & 0.001 & -0.025 & 0.050 & -0.092 & 0.036 & -0.070 & 0.024 & -0.093 & 0.033 & -0.066 & 0.041 & -0.072 & 0.020 & -0.073 & 0.056 & -0.092 & 0.083 & -0.078 & 0.042 & -0.041 & 0.040 & -0.043 & 0.056 & -0.066 & 0.040 & -0.042 & 0.054 &  0.023 & 0.050 & -0.108 & 0.027 \\
 22919 & -0.172 & 0.053 & -0.153 & 0.006 & -0.288 & 0.006 & -0.100 & 0.050 & -0.213 & 0.048 & -0.187 & 0.028 & -0.162 & 0.029 & -0.133 & 0.041 & -0.189 & 0.032 & -0.162 & 0.083 & -0.200 & 0.090 & -0.138 & 0.076 & -0.184 & 0.059 & -0.182 & 0.096 & -0.208 & 0.044 & -0.273 & 0.075 & -0.200 & 0.050 & -0.062 & 0.060 \\
 25388 & -0.226 & 0.059 & -0.187 & 0.010 & -0.323 & 0.013 & -0.104 & 0.050 & -0.199 & 0.038 & -0.202 & 0.030 & -0.234 & 0.057 & -0.164 & 0.037 & -0.179 & 0.004 & -0.180 & 0.054 & -0.209 & 0.060 & -0.208 & 0.033 & -0.263 & 0.034 & -0.171 & 0.073 & -0.242 & 0.037 & -0.311 & 0.063 & -0.224 & 0.050 & -0.138 & 0.054 \\
 27075 & -0.189 & 0.020 & -0.178 & 0.000 & -0.307 & 0.024 & -0.099 & 0.050 & -0.236 & 0.030 & -0.235 & 0.022 & -0.235 & 0.060 & -0.186 & 0.047 & -0.219 & 0.028 & -0.207 & 0.064 & -0.249 & 0.076 & -0.198 & 0.044 & -0.233 & 0.059 & -0.215 & 0.091 & -0.252 & 0.048 & -0.290 & 0.067 & -0.226 & 0.050 & -0.139 & 0.041 \\
 28913 & -0.042 & 0.028 & -0.029 & 0.003 & -0.064 & 0.017 &  0.000 & 0.050 & -0.060 & 0.031 & -0.045 & 0.016 & -0.099 & 0.012 & -0.033 & 0.040 & -0.043 & 0.015 & -0.049 & 0.038 & -0.027 & 0.068 & -0.029 & 0.055 & -0.032 & 0.037 & -0.004 & 0.089 & -0.045 & 0.037 & -0.062 & 0.059 & -0.043 & 0.050 & -0.035 & 0.015 \\
 30711 & -0.222 & 0.025 & -0.194 & 0.013 & -0.331 & 0.040 & -0.147 & 0.050 & -0.205 & 0.046 & -0.215 & 0.028 & -0.257 & 0.014 & -0.165 & 0.038 & -0.199 & 0.005 & -0.163 & 0.082 & -0.187 & 0.064 & -0.210 & 0.029 & -0.285 & 0.052 & -0.165 & 0.032 & -0.233 & 0.036 & -0.326 & 0.088 & -0.256 & 0.050 & -0.109 & 0.058 \\
 37645 & -0.138 & 0.042 & -0.109 & 0.013 & -0.214 & 0.027 & -0.064 & 0.050 & -0.138 & 0.056 & -0.158 & 0.028 & -0.219 & 0.023 & -0.085 & 0.021 & -0.129 & 0.033 & -0.034 & 0.118 & -0.047 & 0.072 & -0.138 & 0.044 & -0.199 & 0.031 & -0.113 & 0.102 & -0.212 & 0.053 & -0.229 & 0.071 & -0.158 & 0.050 & -0.071 & 0.040 \\
 41134 & -0.167 & 0.058 & -0.131 & 0.012 & -0.272 & 0.005 & -0.106 & 0.050 & -0.182 & 0.039 & -0.173 & 0.019 & -0.191 & 0.059 & -0.122 & 0.049 & -0.182 & 0.027 & -0.144 & 0.068 & -0.184 & 0.066 & -0.116 & 0.053 & -0.129 & 0.034 & -0.168 & 0.063 & -0.181 & 0.043 & -0.224 & 0.052 & -0.148 & 0.050 & -0.036 & 0.048 \\
 41226 &  0.017 & 0.044 &  0.029 & 0.012 & -0.061 & 0.006 &  0.023 & 0.050 & -0.067 & 0.031 & -0.022 & 0.019 & -0.055 & 0.073 & -0.026 & 0.041 & -0.034 & 0.003 & -0.027 & 0.077 & -0.028 & 0.060 & -0.017 & 0.064 & -0.018 & 0.057 &  0.004 & 0.079 & -0.038 & 0.045 & -0.027 & 0.025 & -0.002 & 0.050 & -0.027 & 0.015 \\
 41968 & -0.232 & 0.031 & -0.180 & 0.005 & -0.320 & 0.029 & -0.132 & 0.050 & -0.198 & 0.032 & -0.200 & 0.019 & -0.225 & 0.066 & -0.150 & 0.054 & -0.176 & 0.015 & -0.132 & 0.064 & -0.174 & 0.063 & -0.192 & 0.041 & -0.237 & 0.039 & -0.171 & 0.056 & -0.259 & 0.036 & -0.368 & 0.076 & -0.221 & 0.050 & -0.078 & 0.042 \\
 42123 & -0.151 & 0.028 & -0.121 & 0.017 & -0.219 & 0.011 & -0.021 & 0.050 & -0.127 & 0.041 & -0.155 & 0.024 & -0.171 & 0.166 & -0.129 & 0.040 & -0.134 & 0.023 & -0.137 & 0.063 & -0.180 & 0.061 & -0.177 & 0.042 & -0.179 & 0.026 & -0.168 & 0.062 & -0.176 & 0.053 & -0.210 & 0.049 & -0.116 & 0.050 & -0.123 & 0.038 \\
 42723 & -0.106 & 0.046 & -0.096 & 0.009 & -0.140 & 0.013 & -0.041 & 0.050 & -0.095 & 0.043 & -0.128 & 0.014 & -0.186 & 0.110 & -0.114 & 0.029 & -0.110 & 0.026 & -0.101 & 0.071 & -0.135 & 0.064 & -0.134 & 0.031 & -0.104 & 0.033 & -0.091 & 0.098 & -0.133 & 0.042 & -0.120 & 0.078 & -0.089 & 0.050 & -0.135 & 0.043 \\
 48351 & -0.099 & 0.011 & -0.085 & 0.002 & -0.146 & 0.006 & -0.054 & 0.050 & -0.101 & 0.042 & -0.107 & 0.027 & -0.186 & 0.057 & -0.095 & 0.025 & -0.103 & 0.015 & -0.091 & 0.075 & -0.147 & 0.044 & -0.112 & 0.052 & -0.152 & 0.035 & -0.087 & 0.060 & -0.138 & 0.041 & -0.120 & 0.003 & -0.099 & 0.050 & -0.087 & 0.051 \\
 48376 & -0.224 & 0.078 & -0.165 & 0.011 & -0.343 & 0.003 & -0.174 & 0.050 & -0.227 & 0.044 & -0.200 & 0.024 & -0.240 & 0.020 & -0.120 & 0.032 & -0.194 & 0.013 & -0.124 & 0.063 & -0.152 & 0.088 & -0.154 & 0.061 & -0.249 & 0.032 & -0.201 & 0.073 & -0.227 & 0.043 & -0.319 & 0.047 & -0.239 & 0.050 &  0.002 & 0.047 \\
 53196 & -0.081 & 0.069 & -0.059 & 0.010 & -0.172 & 0.026 & -0.054 & 0.050 & -0.135 & 0.023 & -0.108 & 0.024 & -0.163 & 0.091 & -0.107 & 0.048 & -0.097 & 0.015 & -0.087 & 0.061 & -0.132 & 0.045 & -0.102 & 0.036 & -0.121 & 0.041 & -0.095 & 0.064 & -0.120 & 0.037 & -0.138 & 0.022 & -0.097 & 0.050 & -0.097 & 0.047 \\
 54383 & -0.228 & 0.013 & -0.146 & 0.009 & -0.308 & 0.037 & -0.062 & 0.050 & -0.137 & 0.035 & -0.168 & 0.031 & -0.308 & 0.103 & -0.074 & 0.040 & -0.099 & 0.011 & -0.075 & 0.084 & -0.111 & 0.053 & -0.142 & 0.026 & -0.247 & 0.059 & -0.138 & 0.077 & -0.170 & 0.036 & -0.284 & 0.071 & -0.230 & 0.050 &  0.040 & 0.031 \\
 60353 & -0.151 & 0.012 & -0.098 & 0.001 & -0.213 & 0.036 & -0.058 & 0.050 & -0.122 & 0.033 & -0.094 & 0.024 & -0.181 & 0.080 & -0.033 & 0.036 & -0.077 & 0.028 & -0.029 & 0.051 & -0.048 & 0.111 & -0.028 & 0.052 & -0.117 & 0.004 & -0.034 & 0.036 & -0.087 & 0.040 & -0.170 & 0.067 & -0.040 & 0.050 &  0.072 & 0.045 \\
 67408 & -0.151 & 0.048 & -0.146 & 0.006 & -0.280 & 0.010 & -0.114 & 0.050 & -0.213 & 0.029 & -0.216 & 0.024 & -0.245 & 0.135 & -0.208 & 0.038 & -0.196 & 0.032 & -0.179 & 0.051 & -0.225 & 0.052 & -0.222 & 0.032 & -0.240 & 0.069 & -0.173 & 0.069 & -0.236 & 0.044 & -0.257 & 0.066 & -0.194 & 0.050 & -0.168 & 0.044 \\
 70782 & -0.130 & 0.054 & -0.086 & 0.016 & -0.236 & 0.011 & -0.036 & 0.050 & -0.149 & 0.053 & -0.105 & 0.032 & -0.127 & 0.028 & -0.063 & 0.034 & -0.102 & 0.038 & -0.074 & 0.052 & -0.103 & 0.065 & -0.070 & 0.050 & -0.122 & 0.063 & -0.093 & 0.034 & -0.135 & 0.031 & -0.178 & 0.030 & -0.121 & 0.050 &  0.039 & 0.032 \\
 73754 & -0.291 & 0.052 & -0.191 & 0.027 & -0.427 & 0.000 & -0.115 & 0.050 & -0.282 & 0.021 & -0.265 & 0.027 & -0.292 & 0.088 & -0.176 & 0.022 & -0.283 & 0.022 & -0.156 & 0.080 & -0.220 & 0.076 & -0.175 & 0.035 & -0.264 & 0.057 & -0.319 & 0.026 & -0.309 & 0.040 & -0.294 & 0.110 & -0.217 & 0.050 &  0.110 & 0.028 \\
 79346 & -0.193 & 0.032 & -0.123 & 0.007 & -0.242 & 0.016 & -0.078 & 0.050 & -0.157 & 0.034 & -0.155 & 0.024 & -0.155 & 0.083 & -0.080 & 0.032 & -0.156 & 0.021 & -0.073 & 0.068 & -0.138 & 0.077 & -0.065 & 0.053 & -0.130 & 0.023 & -0.144 & 0.082 & -0.171 & 0.044 & -0.199 & 0.048 & -0.141 & 0.050 &  0.099 & 0.070 \\
 81062 & -0.190 & 0.053 & -0.101 & 0.013 & -0.322 & 0.034 & -0.312 & 0.050 & -0.082 & 0.034 & -0.099 & 0.029 & -0.221 & 0.024 &  0.011 & 0.028 & -0.037 & 0.008 &  0.020 & 0.068 & -0.022 & 0.096 & -0.070 & 0.034 & -0.189 & 0.048 & -0.100 & 0.082 & -0.125 & 0.037 & -0.258 & 0.078 & -0.177 & 0.050 &  0.074 & 0.032 \\
 83547 & -0.263 & 0.036 & -0.214 & 0.020 & -0.358 & 0.004 & -0.125 & 0.050 & -0.197 & 0.037 & -0.239 & 0.034 & -0.314 & 0.065 & -0.186 & 0.038 & -0.184 & 0.007 & -0.149 & 0.068 & -0.251 & 0.061 & -0.232 & 0.049 & -0.298 & 0.056 & -0.207 & 0.061 & -0.270 & 0.042 & -0.320 & 0.054 & -0.235 & 0.050 & -0.171 & 0.047 \\
 84827 & -0.056 & 0.051 & -0.064 & 0.010 & -0.071 & 0.028 & -0.013 & 0.050 & -0.062 & 0.045 & -0.052 & 0.021 & -0.044 & 0.100 & -0.059 & 0.020 &  0.004 & 0.019 & -0.053 & 0.058 & -0.040 & 0.065 & -0.033 & 0.049 & -0.088 & 0.021 & -0.072 & 0.058 & -0.050 & 0.042 & -0.092 & 0.100 & -0.081 & 0.050 & -0.013 & 0.038 \\
 84856 & -0.070 & 0.038 & -0.079 & 0.010 & -0.075 & 0.012 &  0.056 & 0.050 & -0.008 & 0.036 & -0.030 & 0.023 & -0.102 & 0.077 & -0.013 & 0.024 & -0.055 & 0.011 & -0.034 & 0.031 & -0.047 & 0.041 & -0.014 & 0.056 & -0.068 & 0.004 & -0.050 & 0.067 & -0.056 & 0.037 & -0.050 & 0.041 & -0.033 & 0.050 & -0.024 & 0.029 \\
 90485 & -0.148 & 0.053 & -0.090 & 0.003 & -0.152 & 0.004 &  0.000 & 0.050 & -0.134 & 0.023 & -0.102 & 0.018 & -0.138 & 0.033 & -0.078 & 0.042 & -0.125 & 0.022 & -0.078 & 0.052 & -0.088 & 0.075 & -0.109 & 0.047 & -0.135 & 0.058 & -0.038 & 0.055 & -0.148 & 0.050 & -0.164 & 0.012 & -0.128 & 0.050 & -0.020 & 0.040 \\
 92233 & -0.126 & 0.006 & -0.157 & 0.014 & -0.196 & 0.014 & -0.016 & 0.050 & -0.163 & 0.022 & -0.176 & 0.017 & -0.151 & 0.102 & -0.170 & 0.011 & -0.151 & 0.019 & -0.155 & 0.088 & -0.207 & 0.056 & -0.187 & 0.064 & -0.186 & 0.040 & -0.133 & 0.102 & -0.191 & 0.042 & -0.132 & 0.035 & -0.145 & 0.050 & -0.161 & 0.034 \\
 94645 & -0.102 & 0.025 & -0.052 & 0.018 & -0.134 & 0.004 & -0.028 & 0.050 & -0.080 & 0.031 & -0.054 & 0.023 & -0.096 & 0.027 & -0.012 & 0.046 & -0.056 & 0.009 &  0.021 & 0.072 & -0.017 & 0.059 &  0.003 & 0.034 & -0.043 & 0.007 &  0.033 & 0.034 & -0.055 & 0.040 & -0.059 & 0.050 & -0.001 & 0.050 &  0.050 & 0.004 \\
 95164 & -0.099 & 0.066 & -0.163 & 0.006 & -0.236 & 0.006 & -0.073 & 0.050 & -0.192 & 0.028 & -0.184 & 0.031 & -0.182 & 0.045 & -0.177 & 0.032 & -0.177 & 0.016 & -0.173 & 0.027 & -0.207 & 0.067 & -0.176 & 0.047 & -0.235 & 0.023 & -0.159 & 0.060 & -0.218 & 0.041 & -0.194 & 0.047 & -0.146 & 0.050 & -0.147 & 0.038 \\
 96078 & -0.148 & 0.027 & -0.150 & 0.009 & -0.272 & 0.007 & -0.167 & 0.050 & -0.269 & 0.041 & -0.228 & 0.022 & -0.236 & 0.038 & -0.233 & 0.031 & -0.227 & 0.014 & -0.237 & 0.031 & -0.263 & 0.095 & -0.240 & 0.025 & -0.268 & 0.061 & -0.209 & 0.049 & -0.276 & 0.031 & -0.220 & 0.007 & -0.196 & 0.050 & -0.207 & 0.045 \\
 97546 & -0.145 & 0.048 & -0.119 & 0.011 & -0.219 & 0.030 & -0.093 & 0.050 & -0.131 & 0.027 & -0.143 & 0.015 & -0.159 & 0.027 & -0.109 & 0.035 & -0.127 & 0.006 & -0.105 & 0.049 & -0.145 & 0.060 & -0.118 & 0.055 & -0.142 & 0.011 & -0.123 & 0.070 & -0.148 & 0.037 & -0.161 & 0.085 & -0.107 & 0.050 & -0.080 & 0.043 \\
 97675 & -0.132 & 0.029 & -0.092 & 0.003 & -0.162 & 0.018 & -0.040 & 0.050 & -0.068 & 0.049 & -0.092 & 0.015 & -0.168 & 0.062 & -0.051 & 0.043 & -0.071 & 0.005 & -0.074 & 0.062 & -0.086 & 0.068 & -0.080 & 0.062 & -0.094 & 0.043 & -0.062 & 0.066 & -0.101 & 0.041 & -0.161 & 0.088 & -0.131 & 0.050 & -0.040 & 0.046 \\
100072 & -0.208 & 0.031 & -0.170 & 0.008 & -0.318 & 0.006 & -0.100 & 0.050 & -0.244 & 0.047 & -0.210 & 0.026 & -0.275 & 0.037 & -0.130 & 0.053 & -0.197 & 0.047 & -0.126 & 0.091 & -0.167 & 0.062 & -0.155 & 0.069 & -0.184 & 0.055 & -0.192 & 0.135 & -0.218 & 0.056 & -0.314 & 0.051 & -0.224 & 0.050 &  0.019 & 0.025 \\
100396 & -0.128 & 0.027 & -0.104 & 0.010 & -0.198 & 0.011 & -0.039 & 0.050 & -0.144 & 0.038 & -0.128 & 0.022 & -0.119 & 0.108 & -0.110 & 0.022 & -0.125 & 0.003 & -0.117 & 0.065 & -0.131 & 0.081 & -0.111 & 0.049 & -0.136 & 0.044 & -0.143 & 0.070 & -0.169 & 0.045 & -0.190 & 0.052 & -0.161 & 0.050 & -0.080 & 0.012 \\
104071 & -0.106 & 0.055 & -0.104 & 0.010 & -0.209 & 0.004 & -0.034 & 0.050 & -0.117 & 0.039 & -0.145 & 0.022 & -0.164 & 0.148 & -0.120 & 0.033 & -0.102 & 0.020 & -0.093 & 0.091 & -0.141 & 0.069 & -0.119 & 0.045 & -0.125 & 0.047 & -0.111 & 0.108 & -0.130 & 0.048 & -0.191 & 0.078 & -0.148 & 0.050 & -0.106 & 0.054 \\
108859 & -0.205 & 0.051 & -0.185 & 0.010 & -0.348 & 0.011 & -0.132 & 0.050 & -0.236 & 0.042 & -0.230 & 0.028 & -0.266 & 0.077 & -0.179 & 0.052 & -0.180 & 0.005 & -0.135 & 0.085 & -0.224 & 0.048 & -0.188 & 0.046 & -0.263 & 0.057 & -0.216 & 0.083 & -0.267 & 0.042 & -0.359 & 0.073 & -0.213 & 0.050 & -0.091 & 0.069 \\
113086 & -0.141 & 0.042 & -0.113 & 0.008 & -0.290 & 0.014 & -0.109 & 0.050 & -0.201 & 0.036 & -0.175 & 0.022 & -0.176 & 0.038 & -0.147 & 0.017 & -0.204 & 0.016 & -0.123 & 0.074 & -0.175 & 0.058 & -0.169 & 0.035 & -0.221 & 0.062 & -0.160 & 0.029 & -0.223 & 0.053 & -0.254 & 0.077 & -0.191 & 0.050 & -0.084 & 0.026 \\
114096 & -0.031 & 0.042 & -0.050 & 0.019 & -0.182 & 0.026 & -0.050 & 0.050 & -0.131 & 0.017 & -0.113 & 0.019 & -0.096 & 0.044 & -0.100 & 0.018 & -0.169 & 0.021 & -0.100 & 0.056 & -0.118 & 0.054 & -0.078 & 0.044 & -0.125 & 0.021 & -0.116 & 0.058 & -0.136 & 0.039 & -0.144 & 0.008 & -0.124 & 0.050 &  0.012 & 0.022 \\
114670 & -0.072 & 0.062 & -0.035 & 0.004 & -0.175 & 0.016 & -0.074 & 0.050 & -0.126 & 0.032 & -0.099 & 0.030 & -0.121 & 0.028 & -0.059 & 0.030 & -0.125 & 0.031 & -0.068 & 0.033 & -0.116 & 0.043 & -0.057 & 0.040 & -0.112 & 0.006 & -0.152 & 0.038 & -0.119 & 0.036 & -0.174 & 0.025 & -0.142 & 0.050 &  0.004 & 0.023 \\
\\ \multicolumn{37}{c}{mr: metal-rich solar analogs} \\ \hline
  1499 & -0.103 & 0.023 & -0.099 & 0.015 & -0.134 & 0.011 & -0.134 & 0.050 & -0.106 & 0.008 & -0.115 & 0.028 & -0.041 & 0.034 & -0.096 & 0.021 & -0.116 & 0.019 & -0.117 & 0.036 & -0.119 & 0.022 & -0.110 & 0.039 & -0.085 & 0.037 & -0.137 & 0.021 & -0.125 & 0.019 & -0.184 & 0.001 & -0.077 & 0.050 & -0.093 & 0.028 \\
  1803 & -0.215 & 0.031 & -0.086 & 0.021 & -0.206 & 0.015 & -0.185 & 0.050 & -0.147 & 0.005 & -0.098 & 0.018 & -0.078 & 0.050 & -0.036 & 0.031 & -0.148 & 0.022 & -0.059 & 0.054 & -0.055 & 0.040 & -0.040 & 0.032 & -0.076 & 0.012 & -0.154 & 0.027 & -0.147 & 0.053 & -0.368 & 0.040 & -0.159 & 0.050 &  0.154 & 0.017 \\
  5176 & -0.130 & 0.030 & -0.121 & 0.015 & -0.148 & 0.004 & -0.150 & 0.050 & -0.148 & 0.002 & -0.117 & 0.008 & -0.048 & 0.028 & -0.075 & 0.028 & -0.149 & 0.008 & -0.122 & 0.037 & -0.113 & 0.034 & -0.133 & 0.035 & -0.104 & 0.028 & -0.143 & 0.020 & -0.143 & 0.035 & -0.293 & 0.027 & -0.111 & 0.050 & -0.081 & 0.031 \\
 12048 & -0.229 & 0.049 & -0.141 & 0.012 & -0.340 & 0.014 & -0.183 & 0.005 & -0.189 & 0.007 & -0.179 & 0.027 & -0.178 & 0.010 & -0.109 & 0.033 & -0.188 & 0.024 & -0.148 & 0.034 & -0.177 & 0.028 & -0.151 & 0.028 & -0.222 & 0.011 & -0.224 & 0.019 & -0.210 & 0.037 & -0.357 & 0.006 & -0.155 & 0.050 & -0.084 & 0.012 \\
 12186 & -0.253 & 0.029 & -0.155 & 0.008 & -0.298 & 0.031 & -0.175 & 0.013 & -0.170 & 0.015 & -0.171 & 0.026 & -0.187 & 0.029 & -0.123 & 0.024 & -0.168 & 0.026 & -0.164 & 0.032 & -0.173 & 0.030 & -0.173 & 0.033 & -0.200 & 0.030 & -0.203 & 0.032 & -0.207 & 0.031 & -0.374 & 0.025 & -0.209 & 0.050 & -0.073 & 0.014 \\
 17054 &  0.156 & 0.034 &  0.108 & 0.022 &  0.234 & 0.013 &  0.120 & 0.050 &  0.164 & 0.013 &  0.157 & 0.017 &  0.195 & 0.052 &  0.082 & 0.029 &  0.199 & 0.016 &  0.123 & 0.025 &  0.148 & 0.018 &  0.107 & 0.035 &  0.133 & 0.007 &  0.175 & 0.019 &  0.173 & 0.018 &  0.222 & 0.021 &  0.194 & 0.050 &  0.056 & 0.044 \\
 17960 & -0.126 & 0.036 & -0.080 & 0.009 & -0.183 & 0.007 & -0.118 & 0.011 & -0.072 & 0.022 & -0.095 & 0.020 & -0.094 & 0.050 & -0.046 & 0.029 & -0.067 & 0.004 & -0.076 & 0.024 & -0.090 & 0.029 & -0.104 & 0.022 & -0.124 & 0.010 & -0.119 & 0.021 & -0.119 & 0.029 & -0.263 & 0.012 & -0.115 & 0.050 & -0.025 & 0.008 \\
 20723 & -0.027 & 0.020 & -0.031 & 0.023 & -0.059 & 0.026 & -0.060 & 0.050 & -0.040 & 0.021 & -0.047 & 0.027 &  0.017 & 0.125 & -0.035 & 0.022 & -0.061 & 0.031 & -0.051 & 0.024 & -0.061 & 0.024 & -0.043 & 0.024 & -0.001 & 0.054 & -0.080 & 0.018 & -0.041 & 0.032 & -0.025 & 0.045 & -0.006 & 0.050 & -0.062 & 0.034 \\
 20741 & -0.244 & 0.032 & -0.102 & 0.028 & -0.263 & 0.008 & -0.162 & 0.015 & -0.192 & 0.013 & -0.149 & 0.024 & -0.078 & 0.070 & -0.051 & 0.024 & -0.184 & 0.023 & -0.101 & 0.042 & -0.085 & 0.044 & -0.083 & 0.032 & -0.105 & 0.021 & -0.188 & 0.017 & -0.176 & 0.042 & -0.395 & 0.023 & -0.226 & 0.050 &  0.070 & 0.037 \\
 21923 & -0.153 & 0.032 & -0.065 & 0.009 & -0.177 & 0.011 & -0.044 & 0.050 & -0.008 & 0.008 & -0.049 & 0.023 & -0.092 & 0.069 &  0.001 & 0.014 & -0.021 & 0.021 & -0.015 & 0.022 & -0.020 & 0.019 & -0.047 & 0.038 & -0.111 & 0.001 & -0.046 & 0.028 & -0.048 & 0.027 & -0.240 & 0.013 & -0.109 & 0.050 &  0.021 & 0.003 \\
 22336 & -0.164 & 0.071 & -0.084 & 0.023 & -0.176 & 0.001 & -0.052 & 0.002 & -0.044 & 0.030 & -0.061 & 0.030 & -0.121 & 0.065 & -0.006 & 0.038 & -0.038 & 0.021 & -0.050 & 0.035 & -0.036 & 0.036 & -0.043 & 0.036 & -0.092 & 0.007 & -0.076 & 0.031 & -0.068 & 0.035 & -0.286 & 0.004 & -0.149 & 0.050 &  0.068 & 0.023 \\
 24681 & -0.189 & 0.044 & -0.112 & 0.016 & -0.234 & 0.030 & -0.173 & 0.011 & -0.173 & 0.013 & -0.170 & 0.027 & -0.145 & 0.026 & -0.127 & 0.024 & -0.169 & 0.021 & -0.187 & 0.030 & -0.184 & 0.031 & -0.164 & 0.040 & -0.177 & 0.032 & -0.200 & 0.033 & -0.210 & 0.030 & -0.316 & 0.015 & -0.139 & 0.050 & -0.098 & 0.037 \\
 26935 & -0.115 & 0.060 & -0.078 & 0.017 & -0.174 & 0.029 & -0.113 & 0.032 & -0.092 & 0.011 & -0.098 & 0.026 & -0.067 & 0.020 & -0.066 & 0.031 & -0.092 & 0.007 & -0.098 & 0.020 & -0.104 & 0.030 & -0.088 & 0.038 & -0.108 & 0.025 & -0.141 & 0.017 & -0.127 & 0.032 & -0.249 & 0.033 & -0.113 & 0.050 & -0.041 & 0.020 \\
 29349 & -0.046 & 0.053 & -0.016 & 0.008 & -0.028 & 0.018 & -0.012 & 0.014 & -0.026 & 0.017 & -0.015 & 0.030 & -0.041 & 0.061 & -0.001 & 0.035 & -0.020 & 0.024 & -0.033 & 0.032 & -0.010 & 0.026 & -0.029 & 0.052 & -0.018 & 0.016 & -0.023 & 0.029 & -0.023 & 0.034 & -0.093 & 0.048 & -0.027 & 0.050 & -0.001 & 0.037 \\
 30243 &  0.021 & 0.026 & -0.026 & 0.013 &  0.071 & 0.008 & -0.005 & 0.028 &  0.028 & 0.010 &  0.022 & 0.028 & -0.015 & 0.019 &  0.027 & 0.032 &  0.010 & 0.018 &  0.018 & 0.032 &  0.038 & 0.020 &  0.015 & 0.033 &  0.046 & 0.049 &  0.034 & 0.017 &  0.039 & 0.017 &  0.038 & 0.033 &  0.038 & 0.050 & -0.043 & 0.047 \\
 30480 & -0.024 & 0.050 & -0.060 & 0.025 & -0.115 & 0.011 & -0.111 & 0.050 & -0.122 & 0.019 & -0.073 & 0.028 & -0.045 & 0.007 & -0.064 & 0.023 & -0.114 & 0.013 & -0.111 & 0.029 & -0.105 & 0.039 & -0.095 & 0.028 & -0.097 & 0.042 & -0.112 & 0.012 & -0.107 & 0.026 & -0.142 & 0.013 & -0.037 & 0.050 &  0.066 & 0.037 \\
 31540 & -0.014 & 0.036 & -0.058 & 0.004 & -0.009 & 0.003 & -0.017 & 0.066 & -0.029 & 0.015 & -0.034 & 0.017 &  0.026 & 0.081 & -0.022 & 0.024 & -0.041 & 0.023 & -0.032 & 0.028 & -0.019 & 0.021 & -0.016 & 0.027 & -0.023 & 0.008 & -0.053 & 0.014 & -0.025 & 0.016 & -0.011 & 0.034 & -0.019 & 0.050 & -0.041 & 0.020 \\
 34879 & -0.103 & 0.019 & -0.052 & 0.030 & -0.050 & 0.001 &  0.014 & 0.050 & -0.037 & 0.028 & -0.010 & 0.024 & -0.029 & 0.028 &  0.026 & 0.017 & -0.021 & 0.031 & -0.021 & 0.030 & -0.004 & 0.035 &  0.003 & 0.016 &  0.027 & 0.025 & -0.045 & 0.020 &  0.000 & 0.027 & -0.153 & 0.001 & -0.038 & 0.050 &  0.044 & 0.012 \\
 37309 &  0.011 & 0.014 &  0.016 & 0.017 &  0.009 & 0.004 &  0.005 & 0.007 & -0.005 & 0.005 &  0.016 & 0.026 &  0.011 & 0.093 &  0.018 & 0.021 &  0.014 & 0.026 & -0.016 & 0.027 &  0.011 & 0.030 &  0.014 & 0.026 &  0.034 & 0.030 & -0.010 & 0.019 &  0.020 & 0.023 & -0.068 & 0.023 &  0.028 & 0.050 &  0.018 & 0.008 \\
 39417 &  0.063 & 0.020 & -0.010 & 0.007 &  0.036 & 0.021 & -0.039 & 0.045 &  0.016 & 0.006 &  0.021 & 0.038 &  0.130 & 0.096 &  0.016 & 0.033 &  0.012 & 0.022 &  0.007 & 0.018 &  0.022 & 0.033 &  0.017 & 0.029 &  0.034 & 0.011 & -0.000 & 0.014 &  0.023 & 0.022 &  0.026 & 0.041 &  0.035 & 0.050 &  0.028 & 0.035 \\
 40761 &  0.001 & 0.016 & -0.010 & 0.002 & -0.011 & 0.004 &  0.008 & 0.017 & -0.002 & 0.013 & -0.002 & 0.012 &  0.002 & 0.092 &  0.007 & 0.022 &  0.000 & 0.025 & -0.016 & 0.025 &  0.001 & 0.023 & -0.022 & 0.029 &  0.007 & 0.025 & -0.012 & 0.024 & -0.008 & 0.021 & -0.082 & 0.014 &  0.015 & 0.050 &  0.004 & 0.004 \\
 40952 & -0.072 & 0.060 & -0.072 & 0.002 & -0.124 & 0.017 & -0.112 & 0.018 & -0.097 & 0.011 & -0.100 & 0.028 & -0.039 & 0.029 & -0.063 & 0.029 & -0.125 & 0.025 & -0.098 & 0.023 & -0.103 & 0.022 & -0.103 & 0.033 & -0.079 & 0.025 & -0.126 & 0.017 & -0.113 & 0.029 & -0.153 & 0.016 & -0.095 & 0.050 & -0.062 & 0.015 \\
 51579 & -0.107 & 0.028 & -0.051 & 0.019 & -0.110 & 0.008 & -0.097 & 0.019 & -0.086 & 0.021 & -0.068 & 0.017 & -0.098 & 0.081 & -0.049 & 0.020 & -0.055 & 0.003 & -0.074 & 0.041 & -0.072 & 0.041 & -0.080 & 0.042 & -0.052 & 0.030 & -0.076 & 0.036 & -0.078 & 0.036 & -0.194 & 0.013 & -0.035 & 0.050 & -0.028 & 0.017 \\
 52409 & -0.060 & 0.016 & -0.051 & 0.006 & -0.025 & 0.013 & -0.029 & 0.039 &  0.003 & 0.011 & -0.004 & 0.018 & -0.033 & 0.034 &  0.028 & 0.027 &  0.014 & 0.016 &  0.018 & 0.030 &  0.030 & 0.040 &  0.011 & 0.012 &  0.025 & 0.007 & -0.031 & 0.023 &  0.007 & 0.023 & -0.043 & 0.038 & -0.032 & 0.050 &  0.028 & 0.004 \\
 57291 & -0.094 & 0.031 & -0.002 & 0.007 & -0.050 & 0.027 &  0.030 & 0.067 &  0.049 & 0.018 &  0.026 & 0.023 &  0.072 & 0.068 &  0.059 & 0.033 &  0.046 & 0.018 &  0.043 & 0.027 &  0.045 & 0.031 &  0.024 & 0.019 &  0.013 & 0.006 & -0.002 & 0.020 &  0.024 & 0.026 & -0.061 & 0.014 & -0.007 & 0.050 &  0.101 & 0.017 \\
 60081 & -0.100 & 0.020 & -0.004 & 0.012 & -0.009 & 0.024 &  0.001 & 0.008 &  0.006 & 0.018 &  0.016 & 0.014 &  0.021 & 0.028 &  0.031 & 0.027 & -0.010 & 0.016 &  0.004 & 0.031 &  0.006 & 0.018 &  0.024 & 0.033 &  0.036 & 0.022 & -0.028 & 0.029 &  0.013 & 0.028 & -0.077 & 0.011 &  0.008 & 0.050 &  0.031 & 0.006 \\
 60370 & -0.273 & 0.049 & -0.131 & 0.009 & -0.303 & 0.021 & -0.189 & 0.050 & -0.200 & 0.005 & -0.154 & 0.023 & -0.171 & 0.112 & -0.062 & 0.021 & -0.188 & 0.018 & -0.123 & 0.044 & -0.111 & 0.042 & -0.098 & 0.046 & -0.114 & 0.042 & -0.195 & 0.023 & -0.188 & 0.047 & -0.428 & 0.034 & -0.238 & 0.050 &  0.095 & 0.022 \\
 61379 & -0.027 & 0.031 & -0.012 & 0.004 &  0.031 & 0.018 & -0.174 & 0.050 &  0.019 & 0.013 &  0.036 & 0.029 & -0.018 & 0.069 &  0.021 & 0.034 &  0.025 & 0.030 &  0.001 & 0.024 &  0.028 & 0.020 &  0.019 & 0.022 &  0.023 & 0.013 &  0.023 & 0.017 &  0.036 & 0.019 &  0.005 & 0.033 &  0.008 & 0.050 &  0.051 & 0.021 \\
 61595 & -0.029 & 0.045 & -0.024 & 0.010 & -0.047 & 0.027 & -0.054 & 0.050 & -0.039 & 0.013 & -0.031 & 0.019 & -0.031 & 0.087 & -0.024 & 0.023 & -0.032 & 0.008 & -0.048 & 0.026 & -0.036 & 0.024 & -0.034 & 0.033 & -0.011 & 0.025 & -0.050 & 0.032 & -0.039 & 0.021 & -0.111 & 0.007 & -0.030 & 0.050 & -0.003 & 0.015 \\
 62345 & -0.033 & 0.011 & -0.036 & 0.015 & -0.044 & 0.025 & -0.028 & 0.008 & -0.027 & 0.008 & -0.023 & 0.020 &  0.031 & 0.042 & -0.006 & 0.017 & -0.040 & 0.024 & -0.028 & 0.016 & -0.022 & 0.017 & -0.018 & 0.039 &  0.009 & 0.040 & -0.041 & 0.014 & -0.026 & 0.019 & -0.075 & 0.027 & -0.019 & 0.050 & -0.009 & 0.011 \\
 65808 & -0.031 & 0.049 & -0.059 & 0.009 & -0.134 & 0.026 & -0.078 & 0.050 & -0.082 & 0.013 & -0.069 & 0.011 & -0.027 & 0.101 & -0.041 & 0.016 & -0.092 & 0.009 & -0.066 & 0.033 & -0.063 & 0.023 & -0.043 & 0.023 & -0.049 & 0.001 & -0.108 & 0.015 & -0.082 & 0.019 & -0.090 & 0.025 & -0.050 & 0.050 & -0.029 & 0.007 \\
 70123 & -0.236 & 0.070 & -0.088 & 0.010 & -0.207 & 0.029 & -0.053 & 0.001 & -0.085 & 0.010 & -0.060 & 0.019 & -0.177 & 0.063 &  0.016 & 0.018 & -0.069 & 0.016 & -0.039 & 0.040 & -0.044 & 0.030 & -0.046 & 0.025 & -0.057 & 0.020 & -0.097 & 0.025 & -0.087 & 0.035 & -0.319 & 0.033 & -0.158 & 0.050 &  0.109 & 0.005 \\
 71803 & -0.041 & 0.031 & -0.056 & 0.013 & -0.045 & 0.024 & -0.047 & 0.014 & -0.046 & 0.007 & -0.031 & 0.015 & -0.071 & 0.057 & -0.015 & 0.039 & -0.019 & 0.019 & -0.046 & 0.032 & -0.024 & 0.025 & -0.017 & 0.039 & -0.011 & 0.023 & -0.048 & 0.011 & -0.027 & 0.024 & -0.115 & 0.016 & -0.010 & 0.050 & -0.023 & 0.010 \\
 73408 & -0.101 & 0.048 & -0.001 & 0.016 & -0.023 & 0.021 & -0.021 & 0.052 &  0.001 & 0.020 &  0.029 & 0.013 & -0.046 & 0.062 &  0.060 & 0.032 & -0.013 & 0.013 &  0.012 & 0.029 &  0.036 & 0.022 &  0.035 & 0.016 &  0.062 & 0.011 & -0.013 & 0.025 &  0.013 & 0.034 & -0.127 & 0.001 & -0.034 & 0.050 &  0.044 & 0.029 \\
 74500 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.000 &  0.000 & 0.050 &  0.000 & 0.000 \\
 77740 & -0.253 & 0.048 & -0.176 & 0.018 & -0.326 & 0.018 & -0.221 & 0.050 & -0.224 & 0.012 & -0.178 & 0.022 & -0.183 & 0.068 & -0.113 & 0.021 & -0.201 & 0.008 & -0.179 & 0.036 & -0.155 & 0.033 & -0.146 & 0.048 & -0.175 & 0.039 & -0.211 & 0.039 & -0.222 & 0.037 & -0.442 & 0.040 & -0.230 & 0.050 & -0.021 & 0.014 \\
 78955 & -0.099 & 0.044 & -0.032 & 0.013 & -0.049 & 0.015 &  0.002 & 0.050 &  0.045 & 0.013 &  0.035 & 0.019 & -0.047 & 0.071 &  0.059 & 0.016 &  0.064 & 0.026 &  0.037 & 0.040 &  0.054 & 0.025 &  0.030 & 0.026 &  0.030 & 0.001 &  0.020 & 0.029 &  0.033 & 0.025 & -0.150 & 0.017 & -0.040 & 0.050 &  0.063 & 0.024 \\
 81022 & -0.066 & 0.056 & -0.025 & 0.012 & -0.059 & 0.004 & -0.028 & 0.071 &  0.012 & 0.027 &  0.015 & 0.022 & -0.054 & 0.063 &  0.045 & 0.032 &  0.013 & 0.014 &  0.012 & 0.032 &  0.036 & 0.028 &  0.022 & 0.026 &  0.012 & 0.019 & -0.009 & 0.033 &  0.008 & 0.040 & -0.149 & 0.040 & -0.031 & 0.050 &  0.071 & 0.034 \\
 81767 & -0.009 & 0.058 &  0.003 & 0.003 &  0.051 & 0.018 &  0.011 & 0.017 &  0.026 & 0.015 &  0.026 & 0.011 &  0.016 & 0.031 &  0.019 & 0.010 &  0.035 & 0.019 &  0.006 & 0.022 &  0.025 & 0.019 &  0.005 & 0.016 &  0.009 & 0.016 &  0.026 & 0.014 &  0.031 & 0.022 &  0.000 & 0.040 &  0.025 & 0.050 &  0.008 & 0.014 \\
 83906 & -0.009 & 0.020 &  0.002 & 0.019 &  0.038 & 0.001 &  0.027 & 0.011 &  0.036 & 0.005 &  0.031 & 0.018 &  0.058 & 0.051 &  0.012 & 0.020 &  0.032 & 0.013 &  0.007 & 0.019 &  0.026 & 0.016 &  0.020 & 0.036 &  0.022 & 0.004 &  0.021 & 0.025 &  0.031 & 0.015 &  0.016 & 0.037 &  0.038 & 0.050 &  0.044 & 0.019 \\
 86796 & -0.026 & 0.035 & -0.015 & 0.015 & -0.007 & 0.025 & -0.021 & 0.051 &  0.008 & 0.008 &  0.009 & 0.013 & -0.004 & 0.049 &  0.017 & 0.018 &  0.007 & 0.023 &  0.004 & 0.029 &  0.008 & 0.019 &  0.006 & 0.011 &  0.021 & 0.014 & -0.013 & 0.020 &  0.001 & 0.020 & -0.040 & 0.016 &  0.018 & 0.050 &  0.043 & 0.019 \\
 90593 & -0.002 & 0.055 & -0.009 & 0.008 &  0.045 & 0.004 &  0.001 & 0.021 &  0.034 & 0.019 &  0.046 & 0.038 & -0.005 & 0.059 &  0.030 & 0.025 &  0.022 & 0.009 &  0.020 & 0.032 &  0.029 & 0.018 &  0.023 & 0.033 &  0.050 & 0.006 &  0.018 & 0.022 &  0.033 & 0.022 &  0.005 & 0.024 &  0.040 & 0.050 & -0.001 & 0.021 \\
 91332 & -0.118 & 0.028 & -0.071 & 0.022 & -0.189 & 0.020 & -0.124 & 0.034 & -0.087 & 0.008 & -0.085 & 0.039 & -0.095 & 0.046 & -0.059 & 0.015 & -0.095 & 0.033 & -0.090 & 0.029 & -0.106 & 0.022 & -0.095 & 0.031 & -0.111 & 0.012 & -0.120 & 0.019 & -0.124 & 0.027 & -0.173 & 0.050 & -0.081 & 0.050 & -0.006 & 0.013 \\
 94256 & -0.030 & 0.023 & -0.024 & 0.019 & -0.072 & 0.017 & -0.017 & 0.018 &  0.001 & 0.012 & -0.007 & 0.010 &  0.057 & 0.024 &  0.004 & 0.015 & -0.012 & 0.020 & -0.017 & 0.029 & -0.019 & 0.018 & -0.021 & 0.031 & -0.044 & 0.000 & -0.028 & 0.021 & -0.042 & 0.025 & -0.052 & 0.000 & -0.019 & 0.050 &  0.020 & 0.003 \\
 95740 & -0.096 & 0.017 & -0.020 & 0.025 & -0.043 & 0.022 & -0.029 & 0.032 & -0.021 & 0.011 &  0.007 & 0.016 & -0.061 & 0.088 &  0.022 & 0.029 &  0.012 & 0.001 & -0.011 & 0.047 &  0.020 & 0.025 &  0.005 & 0.029 &  0.018 & 0.007 & -0.022 & 0.024 &  0.009 & 0.027 & -0.099 & 0.030 &  0.007 & 0.050 &  0.051 & 0.012 \\
 98589 & -0.220 & 0.055 & -0.120 & 0.012 & -0.211 & 0.018 & -0.136 & 0.036 & -0.129 & 0.007 & -0.116 & 0.018 & -0.129 & 0.058 & -0.043 & 0.017 & -0.122 & 0.016 & -0.084 & 0.033 & -0.052 & 0.031 & -0.073 & 0.028 & -0.080 & 0.026 & -0.116 & 0.029 & -0.121 & 0.045 & -0.291 & 0.020 & -0.164 & 0.050 &  0.051 & 0.032 \\
 99115 &  0.052 & 0.043 &  0.033 & 0.014 & -0.125 & 0.023 &  0.017 & 0.057 &  0.033 & 0.013 & -0.006 & 0.019 &  0.040 & 0.044 &  0.008 & 0.014 &  0.022 & 0.001 &  0.036 & 0.028 &  0.003 & 0.032 & -0.028 & 0.028 & -0.095 & 0.001 & -0.034 & 0.013 & -0.041 & 0.018 & -0.039 & 0.009 &  0.044 & 0.050 &  0.040 & 0.037 \\
 99727 & -0.053 & 0.033 & -0.057 & 0.017 & -0.153 & 0.035 & -0.091 & 0.054 & -0.062 & 0.012 & -0.066 & 0.014 & -0.063 & 0.032 & -0.042 & 0.009 & -0.039 & 0.017 & -0.060 & 0.031 & -0.054 & 0.030 & -0.064 & 0.032 & -0.072 & 0.028 & -0.079 & 0.013 & -0.079 & 0.032 & -0.225 & 0.021 & -0.077 & 0.050 & -0.007 & 0.012 \\
 99729 & -0.080 & 0.034 & -0.063 & 0.005 & -0.148 & 0.013 & -0.103 & 0.013 & -0.063 & 0.011 & -0.070 & 0.017 & -0.081 & 0.035 & -0.045 & 0.019 & -0.071 & 0.005 & -0.067 & 0.026 & -0.059 & 0.025 & -0.058 & 0.035 & -0.089 & 0.007 & -0.083 & 0.020 & -0.083 & 0.026 & -0.195 & 0.030 & -0.061 & 0.050 & -0.031 & 0.026 \\
100500 & -0.148 & 0.044 & -0.117 & 0.027 & -0.226 & 0.001 & -0.071 & 0.006 & -0.098 & 0.021 & -0.105 & 0.024 & -0.071 & 0.029 & -0.059 & 0.020 & -0.107 & 0.020 & -0.094 & 0.027 & -0.107 & 0.018 & -0.090 & 0.033 & -0.115 & 0.004 & -0.146 & 0.015 & -0.134 & 0.023 & -0.210 & 0.004 & -0.125 & 0.050 &  0.002 & 0.009 \\
101806 & -0.090 & 0.058 & -0.052 & 0.024 & -0.060 & 0.022 & -0.015 & 0.001 & -0.023 & 0.016 & -0.028 & 0.026 & -0.014 & 0.029 &  0.005 & 0.033 & -0.004 & 0.040 & -0.041 & 0.033 & -0.023 & 0.032 & -0.031 & 0.029 & -0.030 & 0.033 & -0.044 & 0.034 & -0.044 & 0.026 & -0.159 & 0.002 & -0.043 & 0.050 &  0.016 & 0.036 \\
103682 & -0.099 & 0.037 & -0.034 & 0.018 & -0.037 & 0.004 & -0.054 & 0.054 & -0.032 & 0.011 & -0.016 & 0.024 &  0.016 & 0.033 & -0.003 & 0.026 & -0.025 & 0.015 & -0.038 & 0.046 & -0.001 & 0.038 & -0.023 & 0.035 &  0.009 & 0.040 & -0.019 & 0.011 & -0.011 & 0.037 & -0.148 & 0.030 & -0.025 & 0.050 & -0.006 & 0.030 \\
106006 & -0.164 & 0.023 & -0.098 & 0.007 & -0.134 & 0.008 & -0.114 & 0.047 & -0.130 & 0.002 & -0.109 & 0.020 & -0.055 & 0.031 & -0.085 & 0.026 & -0.100 & 0.015 & -0.117 & 0.034 & -0.105 & 0.017 & -0.098 & 0.032 & -0.066 & 0.051 & -0.127 & 0.020 & -0.116 & 0.020 & -0.141 & 0.014 & -0.075 & 0.050 & -0.085 & 0.020 \\
109355 & -0.120 & 0.023 & -0.057 & 0.023 & -0.080 & 0.005 & -0.076 & 0.002 & -0.063 & 0.006 & -0.040 & 0.018 & -0.061 & 0.049 & -0.026 & 0.013 & -0.052 & 0.020 & -0.056 & 0.025 & -0.044 & 0.019 & -0.020 & 0.036 & -0.002 & 0.018 & -0.075 & 0.026 & -0.033 & 0.021 & -0.129 & 0.026 & -0.061 & 0.050 & -0.026 & 0.030 \\
110161 & -0.097 & 0.039 & -0.026 & 0.014 & -0.013 & 0.019 & -0.008 & 0.065 & -0.026 & 0.008 &  0.006 & 0.021 & -0.041 & 0.049 &  0.001 & 0.026 &  0.023 & 0.014 &  0.006 & 0.029 &  0.029 & 0.033 &  0.002 & 0.050 &  0.002 & 0.017 & -0.013 & 0.027 & -0.001 & 0.027 & -0.121 & 0.032 &  0.014 & 0.050 &  0.034 & 0.016 \\
110843 &  0.057 & 0.017 &  0.012 & 0.014 & -0.008 & 0.026 & -0.037 & 0.050 &  0.007 & 0.011 & -0.002 & 0.014 &  0.056 & 0.024 &  0.010 & 0.022 & -0.001 & 0.038 & -0.006 & 0.032 & -0.003 & 0.022 &  0.019 & 0.028 &  0.002 & 0.002 & -0.029 & 0.018 &  0.010 & 0.013 &  0.022 & 0.030 &  0.017 & 0.050 &  0.030 & 0.009 \\
113137 & -0.089 & 0.058 & -0.053 & 0.014 & -0.099 & 0.001 & -0.076 & 0.050 & -0.025 & 0.019 & -0.049 & 0.022 & -0.056 & 0.028 & -0.014 & 0.030 & -0.024 & 0.021 & -0.051 & 0.034 & -0.040 & 0.029 & -0.039 & 0.040 & -0.044 & 0.013 & -0.071 & 0.027 & -0.067 & 0.024 & -0.147 & 0.004 & -0.081 & 0.050 &  0.028 & 0.031 \\
115100 & -0.178 & 0.068 & -0.108 & 0.013 & -0.190 & 0.001 & -0.117 & 0.016 & -0.097 & 0.018 & -0.104 & 0.022 & -0.126 & 0.013 & -0.061 & 0.025 & -0.071 & 0.020 & -0.097 & 0.023 & -0.110 & 0.030 & -0.115 & 0.037 & -0.103 & 0.046 & -0.135 & 0.026 & -0.134 & 0.033 & -0.306 & 0.033 & -0.132 & 0.050 & -0.007 & 0.027 \\
116852 & -0.174 & 0.039 & -0.110 & 0.029 & -0.192 & 0.012 & -0.137 & 0.009 & -0.094 & 0.019 & -0.110 & 0.023 & -0.068 & 0.040 & -0.073 & 0.024 & -0.085 & 0.021 & -0.093 & 0.026 & -0.090 & 0.023 & -0.120 & 0.033 & -0.126 & 0.050 & -0.129 & 0.025 & -0.130 & 0.033 & -0.263 & 0.032 & -0.160 & 0.050 & -0.024 & 0.018 \\


==> agerhk.tex <==
\\ \multicolumn{8}{c}{wm: late F dwarfs} \\ \hline
   522 & 1.26 & 1.22 & 1.29 & 2.60 & 1.95 & 2.99 & -4.98 \\
  3119 & 1.22 & 1.20 & 1.24 & 1.16 & 0.17 & 2.16 & -4.91 \\
  3236 & 1.22 & 1.21 & 1.25 & 0.39 & 0.12 & 1.87 & -4.72 \\
  3540 & 1.22 & 1.16 & 1.26 & 3.82 & 3.67 & 5.01 & -4.91 \\
  5862 & 1.18 & 1.17 & 1.20 & 2.14 & 0.67 & 2.93 & -4.98 \\
  5985 & 1.14 & 1.13 & 1.16 & 1.58 & 0.18 & 2.75 & -4.90 \\
  7978 & 1.12 & 1.11 & 1.14 & 1.92 & 0.35 & 3.25 & -4.82 \\
  8548 & 1.13 & 1.11 & 1.17 & 4.17 & 3.70 & 4.50 & -5.01 \\
 12653 & 1.19 & 1.18 & 1.20 & 0.85 & 0.31 & 1.79 & -4.63 \\
 12764 & 1.19 & 1.18 & 1.20 & 1.85 & 1.22 & 2.70 & -4.97 \\
 14194 & 1.30 & 1.28 & 1.31 & 0.21 & 0.13 & 1.25 & -4.72 \\
 14857 & 1.20 & 1.18 & 1.24 & 3.09 & 2.68 & 3.44 & -5.00 \\
 14954 & 1.31 & 1.27 & 1.35 & 3.19 & 2.98 & 3.31 & -4.95 \\
 17819 & 1.26 & 1.23 & 1.30 & 3.51 & 3.29 & 3.61 & -5.00 \\
 22919 & 1.12 & 1.11 & 1.15 & 3.14 & 1.15 & 3.75 & -4.87 \\
 25388 & 1.15 & 1.13 & 1.20 & 4.00 & 3.86 & 4.29 & -5.01 \\
 27075 & 1.10 & 1.08 & 1.11 & 3.96 & 2.27 & 4.55 & -4.96 \\
 28913 & 1.26 & 1.24 & 1.31 & 2.82 & 2.51 & 3.09 & -4.95 \\
 30711 & 1.20 & 1.15 & 1.24 & 3.58 & 3.31 & 3.73 & -5.01 \\
 37645 & 1.25 & 1.21 & 1.30 & 3.63 & 3.44 & 3.75 & -4.99 \\
 41134 & 1.11 & 1.09 & 1.12 & 2.50 & 0.88 & 3.89 & -4.85 \\
 41226 & 1.25 & 1.23 & 1.28 & 1.34 & 0.43 & 2.33 & -4.97 \\
 41968 & 1.16 & 1.14 & 1.19 & 3.37 & 2.52 & 3.59 & -5.00 \\
 42123 & 1.16 & 1.14 & 1.25 & 4.32 & 4.19 & 5.61 & -5.03 \\
 42723 & 1.18 & 1.14 & 1.22 & 4.32 & 4.01 & 4.53 & -5.00 \\
 48351 & 1.29 & 1.18 & 1.33 & 3.93 & 3.70 & 5.15 & -5.04 \\
 48376 & 1.16 & 1.15 & 1.18 & 2.73 & 0.99 & 3.12 & -4.93 \\
 53196 & 1.15 & 1.14 & 1.18 & 2.95 & 1.86 & 3.58 & -4.99 \\
 54383 & 1.18 & 1.16 & 1.21 & 3.39 & 2.66 & 3.62 & -4.96 \\
 60353 & 1.20 & 1.19 & 1.23 & 1.85 & 0.13 & 2.55 & -4.91 \\
 67408 & 1.12 & 1.11 & 1.14 & 1.87 & 0.54 & 3.23 & -4.86 \\
 70782 & 1.19 & 1.18 & 1.21 & 1.77 & 0.81 & 2.84 & -4.95 \\
 73754 & 1.12 & 1.10 & 1.13 & 0.47 & 0.26 & 2.57 & -4.49 \\
 79346 & 1.12 & 1.10 & 1.12 & 2.50 & 0.94 & 3.71 & -4.64 \\
 81062 & 1.25 & 1.23 & 1.29 & 2.45 & 1.25 & 2.63 & -5.01 \\
 83547 & 1.12 & 1.10 & 1.17 & 4.55 & 4.30 & 5.50 & -4.97 \\
 84827 & 1.25 & 1.21 & 1.28 & 3.59 & 3.43 & 3.70 & -4.87 \\
 84856 & 1.33 & 1.28 & 1.45 & 4.35 & 3.02 & 4.46 & -5.06 \\
 90485 & 1.38 & 1.32 & 1.43 & 2.91 & 2.70 & 3.11 & -5.03 \\
 92233 & 1.19 & 1.16 & 1.22 & 5.30 & 4.96 & 5.59 & -5.05 \\
 94645 & 1.24 & 1.23 & 1.25 & 0.20 & 0.12 & 1.16 & -4.73 \\
 95164 & 1.18 & 1.14 & 1.24 & 4.22 & 4.00 & 5.43 & -4.97 \\
 96078 & 1.14 & 1.12 & 1.22 & 3.76 & 3.27 & 4.01 & -5.00 \\
 97546 & 1.16 & 1.14 & 1.19 & 3.41 & 2.84 & 3.78 & -4.99 \\
 97675 & 1.23 & 1.20 & 1.28 & 3.48 & 3.09 & 3.63 & -4.99 \\
100072 & 1.16 & 1.14 & 1.17 & 0.27 & 0.15 & 2.28 & -4.73 \\
100396 & 1.27 & 1.23 & 1.32 & 3.49 & 3.28 & 3.60 & -5.02 \\
104071 & 1.12 & 1.11 & 1.15 & 3.85 & 2.43 & 4.24 & -4.99 \\
108859 & 1.12 & 1.10 & 1.13 & 0.53 & 0.15 & 2.91 & -4.96 \\
113086 & 1.16 & 1.15 & 1.20 & 2.92 & 2.02 & 3.45 & -4.97 \\
114096 & 1.17 & 1.16 & 1.19 & 2.34 & 0.76 & 3.11 & -4.67 \\
114670 & 1.19 & 1.17 & 1.20 & 2.43 & 0.65 & 2.88 & -4.85 \\
\\ \multicolumn{8}{c}{mr: metal-rich solar analogs} \\ \hline
  1499 & 1.03 & 1.02 & 1.05 & 6.07 & 4.62 & 7.05 & -5.04 \\
  1803 & 1.09 & 1.08 & 1.11 & 0.85 & 0.06 & 1.97 & -4.49 \\
  5176 & 1.08 & 1.06 & 1.10 & 3.94 & 2.61 & 4.77 & -5.02 \\
 12048 & 1.06 & 1.04 & 1.09 & 7.95 & 7.41 & 8.43 & -5.07 \\
 12186 & 1.08 & 1.06 & 1.11 & 7.29 & 6.76 & 7.77 & -5.05 \\
 17054 & 1.20 & 1.16 & 1.21 & 4.41 & 4.12 & 4.53 & -5.07 \\
 17960 & 1.09 & 1.07 & 1.12 & 5.96 & 5.24 & 6.92 & -5.07 \\
 20723 & 1.02 & 1.01 & 1.04 & 6.88 & 5.78 & 7.90 & -5.05 \\
 20741 & 1.08 & 1.06 & 1.10 & 0.84 & 0.04 & 2.04 & -4.45 \\
 21923 & 1.16 & 1.09 & 1.18 & 6.56 & 5.13 & 7.12 & -5.07 \\
 22336 & 1.22 & 1.19 & 1.26 & 4.09 & 3.86 & 4.57 & -5.06 \\
 24681 & 1.06 & 1.04 & 1.09 & 6.95 & 6.44 & 7.66 & -5.04 \\
 26935 & 1.10 & 1.08 & 1.14 & 6.25 & 5.01 & 6.79 & -5.08 \\
 29349 & 1.20 & 1.17 & 1.22 & 4.18 & 3.99 & 4.46 & -5.02 \\
 30243 & 1.12 & 1.10 & 1.13 & 4.42 & 3.68 & 4.77 & -5.03 \\
 30480 & 1.16 & 1.12 & 1.19 & 4.86 & 4.30 & 6.02 & -5.07 \\
 31540 & 1.05 & 1.04 & 1.06 & 5.84 & 5.25 & 6.29 & -5.05 \\
 34879 & 1.14 & 1.12 & 1.15 & 2.86 & 1.11 & 3.57 & -5.00 \\
 37309 & 1.11 & 1.09 & 1.13 & 4.35 & 3.37 & 4.64 & -5.06 \\
 39417 & 1.07 & 1.06 & 1.08 & 5.19 & 4.54 & 5.54 & -5.06 \\
 40761 & 1.12 & 1.10 & 1.15 & 4.51 & 3.88 & 4.63 & -5.07 \\
 40952 & 1.01 & 1.00 & 1.03 & 5.86 & 4.86 & 7.14 & -4.98 \\
 51579 & 1.12 & 1.11 & 1.15 & 4.02 & 3.07 & 4.40 & -5.08 \\
 52409 & 1.08 & 1.07 & 1.09 & 4.45 & 3.42 & 5.13 & -5.04 \\
 57291 & 1.10 & 1.08 & 1.11 & 5.80 & 5.65 & 6.12 & -5.06 \\
 60081 & 1.09 & 1.08 & 1.11 & 4.95 & 4.07 & 5.10 & -5.03 \\
 60370 & 1.09 & 1.07 & 1.11 & 1.43 & 0.29 & 3.31 & -4.73 \\
 61379 & 1.17 & 1.15 & 1.30 & 5.86 & 4.08 & 6.20 & -5.11 \\
 61595 & 1.12 & 1.10 & 1.15 & 4.41 & 3.64 & 4.63 & -5.07 \\
 62345 & 1.10 & 1.10 & 1.13 & 5.20 & 5.00 & 5.50 & -5.06 \\
 65808 & 1.04 & 1.03 & 1.06 & 6.65 & 5.94 & 7.76 & -5.05 \\
 70123 & 1.12 & 1.10 & 1.13 & 1.55 & 0.41 & 3.28 & -4.95 \\
 71803 & 1.09 & 1.08 & 1.10 & 3.26 & 1.75 & 3.98 & -5.02 \\
 73408 & 1.12 & 1.11 & 1.14 & 2.65 & 1.24 & 3.76 & -4.88 \\
 74500 & 1.10 & 1.09 & 1.13 & 5.21 & 4.91 & 5.58 & -5.07 \\
 77740 & 1.08 & 1.06 & 1.10 & 1.14 & 0.18 & 2.67 & -4.91 \\
 78955 & 1.15 & 1.13 & 1.19 & 3.97 & 3.49 & 4.38 & -5.06 \\
 81022 & 1.24 & 1.20 & 1.27 & 4.02 & 3.78 & 4.22 & -5.03 \\
 81767 & 1.13 & 1.12 & 1.16 & 4.70 & 4.43 & 4.91 & -5.04 \\
 83906 & 1.22 & 1.14 & 1.26 & 5.23 & 4.58 & 6.59 & -5.11 \\
 86796 & 1.15 & 1.14 & 1.17 & 5.09 & 4.94 & 5.29 & -5.07 \\
 90593 & 1.16 & 1.13 & 1.17 & 4.81 & 4.62 & 4.93 & -5.06 \\
 91332 & 1.08 & 1.06 & 1.10 & 7.72 & 7.27 & 8.26 & -5.06 \\
 94256 & 1.12 & 1.10 & 1.15 & 7.38 & 6.90 & 7.79 & -5.06 \\
 95740 & 1.15 & 1.13 & 1.16 & 2.78 & 1.49 & 3.47 & -5.05 \\
 98589 & 1.12 & 1.08 & 1.12 & 0.43 & 0.30 & 2.20 & -4.78 \\
 99115 & 1.04 & 1.03 & 1.06 & 8.87 & 8.59 & 9.25 & -5.09 \\
 99727 & 1.12 & 1.09 & 1.15 & 5.44 & 5.12 & 6.75 & -5.08 \\
 99729 & 1.10 & 1.08 & 1.12 & 7.70 & 7.33 & 8.07 & -5.09 \\
100500 & 1.09 & 1.08 & 1.11 & 8.12 & 7.72 & 8.43 & -5.09 \\
101806 & 1.13 & 1.11 & 1.16 & 4.16 & 3.44 & 4.49 & -5.07 \\
103682 & 1.15 & 1.13 & 1.17 & 3.05 & 2.09 & 3.72 & -5.04 \\
106006 & 1.04 & 1.03 & 1.06 & 4.94 & 3.53 & 5.55 & -5.05 \\
109355 & 1.07 & 1.05 & 1.08 & 5.06 & 3.63 & 5.35 & -4.99 \\
110161 & 1.16 & 1.14 & 1.19 & 3.48 & 2.76 & 3.92 & -5.03 \\
110843 & 1.07 & 1.06 & 1.09 & 6.02 & 5.79 & 6.60 & -5.07 \\
113137 & 1.17 & 1.12 & 1.20 & 4.68 & 4.46 & 6.17 & -5.09 \\
115100 & 1.12 & 1.10 & 1.20 & 6.26 & 4.82 & 6.66 & -5.09 \\
116852 & 1.09 & 1.08 & 1.14 & 6.56 & 5.26 & 7.03 & -5.04 \\


==> ll.tex <==
 Fe I & 1334 & 5775.0801 & 4.220 & -1.300 \\
 Fe I &      & 5778.4531 & 2.588 & -3.440 \\
 Fe I &      & 5793.9141 & 4.220 & -1.619 \\
 Fe I &      & 5806.7300 & 4.610 & -0.950 \\
 Fe I &      & 5809.2178 & 3.883 & -1.710 \\
 Fe I &      & 5852.2202 & 4.550 & -1.230 \\
 Fe I &      & 5855.0762 & 4.608 & -1.478 \\
 Fe I &      & 5856.0898 & 4.290 & -1.460 \\
 Fe I &      & 5905.6699 & 4.650 & -0.690 \\
 Fe I &      & 5927.7900 & 4.650 & -0.990 \\
 Fe I &      & 5929.6802 & 4.550 & -1.310 \\
 Fe I &      & 5930.1802 & 4.650 & -0.170 \\
 Fe I &      & 5934.6499 & 3.930 & -1.070 \\
 Fe I &      & 5956.6938 & 0.859 & -4.552 \\
 Fe I &      & 6003.0098 & 3.880 & -1.060 \\
 Fe I &      & 6027.0498 & 4.076 & -1.090 \\
 Fe I &      & 6056.0000 & 4.730 & -0.400 \\
 Fe I &      & 6065.4819 & 2.609 & -1.530 \\
 Fe I &      & 6079.0098 & 4.650 & -1.020 \\
 Fe I &      & 6085.2598 & 2.760 & -3.050 \\
 Fe I &      & 6093.6440 & 4.607 & -1.300 \\
 Fe I &      & 6096.6650 & 3.984 & -1.810 \\
 Fe I &      & 6151.6182 & 2.176 & -3.282 \\
 Fe I &      & 6165.3599 & 4.143 & -1.460 \\
 Fe I &      & 6173.3350 & 2.223 & -2.880 \\
 Fe I &      & 6187.9902 & 3.940 & -1.620 \\
 Fe I &      & 6200.3130 & 2.609 & -2.416 \\
 Fe I &      & 6213.4302 & 2.223 & -2.520 \\
 Fe I &      & 6240.6460 & 2.223 & -3.287 \\
 Fe I &      & 6252.5552 & 2.404 & -1.687 \\
 Fe I &      & 6265.1338 & 2.176 & -2.547 \\
 Fe I &      & 6270.2251 & 2.858 & -2.540 \\
 Fe I &      & 6322.6899 & 2.590 & -2.430 \\
 Fe I &      & 6344.1499 & 2.430 & -2.920 \\
 Fe I &      & 6430.8462 & 2.176 & -2.006 \\
 Fe I &      & 6498.9390 & 0.958 & -4.695 \\
 Fe I &      & 6574.2290 & 0.990 & -5.010 \\
 Fe I &      & 6593.8711 & 2.433 & -2.394 \\
 Fe I &      & 6597.5601 & 4.800 & -0.970 \\
 Fe I &      & 6699.1421 & 4.593 & -2.101 \\
 Fe I &      & 6703.5669 & 2.759 & -3.023 \\
 Fe I &      & 6705.1021 & 4.607 & -0.980 \\
 Fe I &      & 6713.7451 & 4.795 & -1.400 \\
 Fe I &      & 6726.6670 & 4.607 & -1.030 \\
 Fe I &      & 6739.5220 & 1.557 & -4.794 \\
 Fe I &      & 6750.1519 & 2.424 & -2.621 \\
 Fe I &      & 6793.2588 & 4.076 & -2.326 \\
 Fe I &      & 6810.2632 & 4.607 & -0.986 \\
 Fe I &      & 6828.5898 & 4.640 & -0.820 \\
 Fe I &      & 6837.0059 & 4.593 & -1.687 \\
 Fe I &      & 6842.6899 & 4.640 & -1.220 \\
 Fe I &      & 6843.6602 & 4.550 & -0.830 \\
 Fe I &      & 6858.1499 & 4.610 & -0.940 \\
 Fe I &      & 6945.2051 & 2.424 & -2.454 \\
 Fe I &      & 6999.8799 & 4.100 & -1.460 \\
 Fe I &      & 7090.3799 & 4.230 & -1.110 \\
 Fe I &      & 7132.9902 & 4.080 & -1.650 \\
 Fe I &      & 7401.6851 & 4.186 & -1.500 \\
 Fe I &      & 7418.6699 & 4.140 & -1.380 \\
Fe II & 1334 & 4491.3999 & 2.856 & -2.660 \\
Fe II &      & 4508.2900 & 2.856 & -2.520 \\
Fe II &      & 6369.4619 & 2.891 & -4.110 \\
Fe II &      & 6432.6758 & 2.891 & -3.570 \\
Fe II &      & 6516.0771 & 2.891 & -3.310 \\
Fe II &      & 7222.3921 & 3.889 & -3.260 \\
Fe II &      & 7515.8311 & 3.903 & -3.390 \\
Fe II &      & 7711.7212 & 3.903 & -2.500 \\
  C I &   40 & 6587.6099 & 8.537 & -1.021 \\
  C I &      & 7111.4692 & 8.640 & -1.074 \\
  C I &      & 7113.1792 & 8.647 & -0.762 \\
  C I &      & 7115.1699 & 8.650 & -0.930 \\
  C I &      & 7116.9600 & 8.650 & -0.910 \\
  O I &  180 & 7771.9438 & 9.146 &  0.352 \\
  O I &      & 7774.1611 & 9.146 &  0.223 \\
  O I &      & 7775.3901 & 9.146 &  0.002 \\
 Na I &  958 & 6154.2251 & 2.102 & -1.547 \\
 Na I &      & 6160.7471 & 2.104 & -1.246 \\
 Mg I & 1336 & 6318.7168 & 5.108 & -1.945 \\
 Mg I &      & 6319.2368 & 5.108 & -2.324 \\
 Al I & 1653 & 6696.0181 & 3.143 & -1.481 \\
 Al I &      & 6698.6670 & 3.143 & -1.782 \\
 Al I &      & 7835.3091 & 4.022 & -0.689 \\
 Al I &      & 7836.1338 & 4.021 & -0.450 \\
 Si I & 1310 & 5772.1450 & 5.082 & -1.653 \\
 Si I &      & 5793.0732 & 4.930 & -1.963 \\
 Si I &      & 5948.5400 & 5.080 & -1.208 \\
 Si I &      & 6125.0298 & 5.610 & -1.510 \\
 Si I &      & 6142.4902 & 5.620 & -1.540 \\
 Si I &      & 6145.0200 & 5.610 & -1.480 \\
 Si I &      & 6195.4600 & 5.870 & -1.666 \\
 Si I &      & 6237.3301 & 5.610 & -1.116 \\
 Si I &      & 6243.8198 & 5.620 & -1.310 \\
 Si I &      & 6244.4800 & 5.610 & -1.360 \\
 Si I &      & 6721.8398 & 5.863 & -1.060 \\
 Si I &      & 6741.6401 & 5.984 & -1.653 \\
 Si I &      & 7405.7700 & 5.614 & -0.720 \\
  S I &  664 & 6046.0000 & 7.868 & -0.100 \\
  S I &      & 6052.6558 & 7.870 & -0.400 \\
  S I &      & 6757.1709 & 7.870 & -0.353 \\
 Ca I & 1517 & 4512.2681 & 2.526 & -1.901 \\
 Ca I &      & 5867.5620 & 2.933 & -1.570 \\
 Ca I &      & 6156.0200 & 2.520 & -2.497 \\
 Ca I &      & 6166.4390 & 2.521 & -1.142 \\
 Ca I &      & 6169.0420 & 2.523 & -0.797 \\
 Ca I &      & 6169.5498 & 2.520 & -0.580 \\
 Ca I &      & 6455.5981 & 2.523 & -1.340 \\
 Ca I &      & 6471.6621 & 2.526 & -0.686 \\
 Ca I &      & 6499.6499 & 2.523 & -0.818 \\
Sc II & 1659 & 6245.6411 & 1.507 & -1.036 \\
Sc II &      & 6320.8428 & 1.500 & -1.923 \\
Sc II &      & 6604.5781 & 1.357 & -1.309 \\
 Ti I & 1582 & 4512.7329 & 0.840 & -0.420 \\
 Ti I &      & 5766.3301 & 3.290 &  0.326 \\
 Ti I &      & 5866.4521 & 1.066 & -0.840 \\
 Ti I &      & 5978.5498 & 1.870 & -0.602 \\
 Ti I &      & 6064.6299 & 1.050 & -1.959 \\
 Ti I &      & 6091.1802 & 2.267 & -0.370 \\
 Ti I &      & 6126.2168 & 1.066 & -1.424 \\
 Ti I &      & 6258.0991 & 1.443 & -0.299 \\
 Ti I &      & 6261.1011 & 1.429 & -0.479 \\
 Ti I &      & 6303.7529 & 1.443 & -1.509 \\
 Ti I &      & 6312.2339 & 1.460 & -1.496 \\
 Ti I &      & 6599.1040 & 0.900 & -2.029 \\
 Ti I &      & 6743.1299 & 0.899 & -1.630 \\
 Ti I &      & 7357.7261 & 1.443 & -1.066 \\
 Ti I &      & 7949.1499 & 1.500 & -1.456 \\
 Ti I &      & 8426.5039 & 0.826 & -1.194 \\
 Ti I &      & 8435.6484 & 0.836 & -0.967 \\
 Ti I &      & 8675.3711 & 1.067 & -1.620 \\
 Ti I &      & 8682.9785 & 1.053 & -1.886 \\
  V I & 1429 & 6039.7271 & 1.063 & -1.854 \\
      &      & 6039.7290 &       & -1.854 \\
      &      & 6039.7300 &       & -2.030 \\
      &      & 6039.7329 &       & -1.690 \\
      &      & 6039.7329 &       & -2.155 \\
      &      & 6039.7339 &       & -2.280 \\
      &      & 6039.7378 &       & -1.682 \\
      &      & 6039.7378 &       & -1.716 \\
      &      & 6039.7388 &       & -2.708 \\
      &      & 6039.7441 &       & -1.843 \\
      &      & 6039.7441 &       & -1.433 \\
      &      & 6039.7510 &       & -1.217 \\
  V I &      & 6081.4170 & 1.051 & -1.660 \\
      &      & 6081.4170 &       & -1.484 \\
      &      & 6081.4268 &       & -1.484 \\
      &      & 6081.4282 &       & -1.359 \\
      &      & 6081.4419 &       & -1.359 \\
      &      & 6081.4419 &       & -1.677 \\
      &      & 6081.4419 &       & -1.472 \\
      &      & 6081.4600 &       & -1.472 \\
  V I &      & 6090.1992 & 1.080 & -0.692 \\
      &      & 6090.2070 &       & -0.833 \\
      &      & 6090.2129 &       & -0.997 \\
      &      & 6090.2129 &       & -1.532 \\
      &      & 6090.2178 &       & -1.195 \\
      &      & 6090.2178 &       & -1.336 \\
      &      & 6090.2231 &       & -1.450 \\
      &      & 6090.2231 &       & -1.282 \\
      &      & 6090.2251 &       & -2.646 \\
      &      & 6090.2261 &       & -1.304 \\
      &      & 6090.2271 &       & -1.838 \\
      &      & 6090.2280 &       & -2.236 \\
      &      & 6090.2290 &       & -1.394 \\
      &      & 6090.2310 &       & -1.583 \\
      &      & 6090.2310 &       & -2.014 \\
      &      & 6090.2319 &       & -1.889 \\
      &      & 6090.2329 &       & -1.868 \\
      &      & 6090.2329 &       & -1.838 \\
  V I &      & 6111.6499 & 1.043 & -0.714 \\
  V I &      & 6119.5098 & 1.064 & -1.825 \\
      &      & 6119.5142 &       & -1.386 \\
      &      & 6119.5161 &       & -1.524 \\
      &      & 6119.5190 &       & -1.524 \\
      &      & 6119.5190 &       & -1.103 \\
      &      & 6119.5210 &       & -1.360 \\
      &      & 6119.5269 &       & -1.700 \\
      &      & 6119.5269 &       & -0.887 \\
      &      & 6119.5278 &       & -1.352 \\
      &      & 6119.5352 &       & -1.950 \\
      &      & 6119.5371 &       & -1.513 \\
      &      & 6119.5459 &       & -2.378 \\
  V I &      & 6135.3418 & 1.051 & -1.552 \\
      &      & 6135.3418 &       & -1.531 \\
      &      & 6135.3428 &       & -1.677 \\
      &      & 6135.3818 &       & -2.008 \\
      &      & 6135.3818 &       & -1.531 \\
      &      & 6135.3833 &       & -1.210 \\
  V I &      & 6199.1548 & 0.286 & -1.958 \\
      &      & 6199.1729 &       & -2.063 \\
      &      & 6199.1880 &       & -2.179 \\
      &      & 6199.2031 &       & -2.308 \\
      &      & 6199.2070 &       & -2.966 \\
      &      & 6199.2148 &       & -2.454 \\
      &      & 6199.2178 &       & -2.755 \\
      &      & 6199.2261 &       & -2.624 \\
      &      & 6199.2271 &       & -2.682 \\
      &      & 6199.2349 &       & -2.676 \\
      &      & 6199.2358 &       & -2.828 \\
      &      & 6199.2412 &       & -2.723 \\
      &      & 6199.2441 &       & -3.091 \\
      &      & 6199.2461 &       & -2.828 \\
      &      & 6199.2490 &       & -3.024 \\
      &      & 6199.2520 &       & -4.267 \\
      &      & 6199.2559 &       & -3.869 \\
      &      & 6199.2588 &       & -3.723 \\
      &      & 6199.2588 &       & -3.665 \\
      &      & 6199.2598 &       & -3.568 \\
      &      & 6199.2612 &       & -3.568 \\
  V I &      & 6216.3252 & 0.275 & -1.460 \\
      &      & 6216.3428 &       & -1.601 \\
      &      & 6216.3579 &       & -1.765 \\
      &      & 6216.3721 &       & -2.300 \\
      &      & 6216.3721 &       & -1.963 \\
      &      & 6216.3828 &       & -2.104 \\
      &      & 6216.3843 &       & -2.218 \\
      &      & 6216.3921 &       & -2.050 \\
      &      & 6216.3955 &       & -2.606 \\
      &      & 6216.3989 &       & -2.072 \\
      &      & 6216.4038 &       & -2.163 \\
      &      & 6216.4082 &       & -2.351 \\
      &      & 6216.4111 &       & -3.414 \\
      &      & 6216.4150 &       & -2.636 \\
      &      & 6216.4160 &       & -3.004 \\
      &      & 6216.4180 &       & -2.606 \\
      &      & 6216.4180 &       & -2.782 \\
      &      & 6216.4189 &       & -2.657 \\
  V I &      & 6224.4609 & 0.287 & -3.519 \\
      &      & 6224.4707 &       & -3.315 \\
      &      & 6224.4800 &       & -3.250 \\
      &      & 6224.4893 &       & -3.257 \\
      &      & 6224.4961 &       & -2.616 \\
      &      & 6224.4961 &       & -3.323 \\
      &      & 6224.5010 &       & -2.803 \\
      &      & 6224.5029 &       & -3.461 \\
      &      & 6224.5049 &       & -3.022 \\
      &      & 6224.5078 &       & -3.285 \\
      &      & 6224.5098 &       & -3.741 \\
      &      & 6224.5112 &       & -3.616 \\
      &      & 6224.5127 &       & -4.063 \\
      &      & 6224.5146 &       & -4.762 \\
      &      & 6224.5205 &       & -3.741 \\
      &      & 6224.5239 &       & -3.461 \\
      &      & 6224.5283 &       & -3.323 \\
      &      & 6224.5312 &       & -3.257 \\
      &      & 6224.5332 &       & -3.250 \\
      &      & 6224.5342 &       & -3.315 \\
      &      & 6224.5352 &       & -3.519 \\
  V I &      & 6242.7979 & 0.262 & -2.017 \\
      &      & 6242.7979 &       & -2.484 \\
      &      & 6242.8291 &       & -2.338 \\
      &      & 6242.8369 &       & -2.338 \\
      &      & 6242.8521 &       & -2.359 \\
      &      & 6242.8682 &       & -2.815 \\
  V I &      & 6243.0449 & 0.301 & -2.751 \\
      &      & 6243.0610 &       & -2.536 \\
      &      & 6243.0752 &       & -2.459 \\
      &      & 6243.0869 &       & -2.448 \\
      &      & 6243.0879 &       & -1.688 \\
      &      & 6243.0981 &       & -1.824 \\
      &      & 6243.0986 &       & -2.491 \\
      &      & 6243.1060 &       & -1.972 \\
      &      & 6243.1094 &       & -2.594 \\
      &      & 6243.1143 &       & -2.131 \\
      &      & 6243.1191 &       & -2.815 \\
      &      & 6243.1201 &       & -2.300 \\
      &      & 6243.1250 &       & -2.467 \\
      &      & 6243.1294 &       & -2.605 \\
      &      & 6243.1318 &       & -2.619 \\
      &      & 6243.1401 &       & -2.751 \\
      &      & 6243.1421 &       & -2.815 \\
      &      & 6243.1426 &       & -2.536 \\
      &      & 6243.1450 &       & -2.594 \\
      &      & 6243.1455 &       & -2.491 \\
      &      & 6243.1455 &       & -2.459 \\
      &      & 6243.1470 &       & -2.448 \\
  V I &      & 6251.7710 & 0.286 & -2.924 \\
      &      & 6251.7881 &       & -2.720 \\
      &      & 6251.8042 &       & -2.655 \\
      &      & 6251.8062 &       & -2.021 \\
      &      & 6251.8169 &       & -2.662 \\
      &      & 6251.8179 &       & -2.208 \\
      &      & 6251.8291 &       & -2.728 \\
      &      & 6251.8291 &       & -2.427 \\
      &      & 6251.8369 &       & -2.690 \\
      &      & 6251.8389 &       & -2.866 \\
      &      & 6251.8442 &       & -3.021 \\
      &      & 6251.8481 &       & -3.146 \\
      &      & 6251.8491 &       & -3.468 \\
      &      & 6251.8530 &       & -4.167 \\
      &      & 6251.8530 &       & -2.924 \\
      &      & 6251.8589 &       & -3.146 \\
      &      & 6251.8589 &       & -2.720 \\
      &      & 6251.8618 &       & -2.655 \\
      &      & 6251.8628 &       & -2.866 \\
      &      & 6251.8638 &       & -2.728 \\
      &      & 6251.8638 &       & -2.662 \\
  V I &      & 6274.6069 & 0.267 & -2.932 \\
      &      & 6274.6289 &       & -2.455 \\
      &      & 6274.6411 &       & -2.476 \\
      &      & 6274.6548 &       & -2.134 \\
      &      & 6274.6572 &       & -2.455 \\
      &      & 6274.6782 &       & -2.601 \\
  V I &      & 6285.0981 & 0.275 & -3.568 \\
      &      & 6285.1172 &       & -3.140 \\
      &      & 6285.1221 &       & -2.703 \\
      &      & 6285.1338 &       & -2.890 \\
      &      & 6285.1372 &       & -2.542 \\
      &      & 6285.1479 &       & -2.714 \\
      &      & 6285.1489 &       & -2.550 \\
      &      & 6285.1519 &       & -2.077 \\
      &      & 6285.1572 &       & -2.714 \\
      &      & 6285.1621 &       & -2.293 \\
      &      & 6285.1680 &       & -2.576 \\
      &      & 6285.1719 &       & -3.015 \\
  V I &      & 6292.7583 & 0.287 & -4.055 \\
      &      & 6292.7759 &       & -3.645 \\
      &      & 6292.7886 &       & -2.941 \\
      &      & 6292.7910 &       & -3.423 \\
      &      & 6292.8008 &       & -2.745 \\
      &      & 6292.8037 &       & -3.298 \\
      &      & 6292.8115 &       & -2.691 \\
      &      & 6292.8164 &       & -3.247 \\
      &      & 6292.8193 &       & -2.713 \\
      &      & 6292.8242 &       & -2.101 \\
      &      & 6292.8247 &       & -3.277 \\
      &      & 6292.8262 &       & -2.804 \\
      &      & 6292.8301 &       & -2.992 \\
      &      & 6292.8311 &       & -2.242 \\
      &      & 6292.8369 &       & -2.406 \\
      &      & 6292.8398 &       & -3.247 \\
      &      & 6292.8398 &       & -2.604 \\
      &      & 6292.8413 &       & -2.859 \\
  V I &      & 6531.3877 & 1.218 & -2.487 \\
      &      & 6531.3911 &       & -2.232 \\
      &      & 6531.3940 &       & -4.140 \\
      &      & 6531.3975 &       & -2.033 \\
      &      & 6531.3989 &       & -2.033 \\
      &      & 6531.4033 &       & -2.897 \\
      &      & 6531.4082 &       & -1.969 \\
      &      & 6531.4092 &       & -1.969 \\
      &      & 6531.4141 &       & -2.180 \\
      &      & 6531.4209 &       & -2.000 \\
      &      & 6531.4219 &       & -2.000 \\
      &      & 6531.4287 &       & -1.774 \\
      &      & 6531.4360 &       & -2.181 \\
      &      & 6531.4380 &       & -2.181 \\
      &      & 6531.4458 &       & -1.482 \\
 Cr I & 1296 & 4511.8999 & 3.090 & -0.390 \\
 Cr I &      & 5783.0732 & 3.232 & -0.480 \\
 Cr I &      & 5783.8701 & 3.322 & -0.290 \\
 Cr I &      & 5787.9302 & 3.322 & -0.080 \\
 Cr I &      & 5844.5918 & 3.013 & -1.770 \\
 Cr I &      & 6330.1001 & 0.941 & -2.900 \\
 Cr I &      & 6661.0801 & 4.190 & -0.234 \\
 Cr I &      & 6882.4771 & 3.438 & -0.375 \\
 Cr I &      & 6882.9971 & 3.438 & -0.420 \\
 Mn I & 1158 & 4502.2041 & 2.920 & -0.610 \\
      &      & 4502.2070 &       & -1.528 \\
      &      & 4502.2080 &       & -2.745 \\
      &      & 4502.2109 &       & -0.750 \\
      &      & 4502.2129 &       & -2.393 \\
      &      & 4502.2129 &       & -1.352 \\
      &      & 4502.2158 &       & -0.908 \\
      &      & 4502.2173 &       & -1.326 \\
      &      & 4502.2178 &       & -2.268 \\
      &      & 4502.2197 &       & -2.347 \\
      &      & 4502.2197 &       & -1.393 \\
      &      & 4502.2197 &       & -1.092 \\
      &      & 4502.2222 &       & -1.569 \\
      &      & 4502.2222 &       & -1.314 \\
      &      & 4502.2227 &       & -1.599 \\
 Mn I &      & 6021.7461 & 3.075 & -2.668 \\
      &      & 6021.7720 &       & -1.451 \\
      &      & 6021.7739 &       & -2.316 \\
      &      & 6021.7949 &       & -1.275 \\
      &      & 6021.7979 &       & -2.191 \\
      &      & 6021.8042 &       & -0.533 \\
      &      & 6021.8130 &       & -1.249 \\
      &      & 6021.8169 &       & -2.271 \\
      &      & 6021.8208 &       & -0.673 \\
      &      & 6021.8271 &       & -1.316 \\
      &      & 6021.8340 &       & -0.831 \\
      &      & 6021.8369 &       & -1.492 \\
      &      & 6021.8428 &       & -1.015 \\
      &      & 6021.8462 &       & -1.522 \\
      &      & 6021.8472 &       & -1.237 \\
      &      & 6082.3149 &       & -2.356 \\
      &      & 6082.3198 &       & -2.135 \\
      &      & 6082.3247 &       & -2.160 \\
      &      & 6082.3296 &       & -2.032 \\
      &      & 6082.3350 &       & -2.146 \\
      &      & 6082.3447 &       & -2.356 \\
      &      & 6082.3462 &       & -1.989 \\
      &      & 6082.3496 &       & -2.008 \\
      &      & 6082.3652 &       & -2.135 \\
      &      & 6082.3657 &       & -2.000 \\
      &      & 6082.3711 &       & -1.841 \\
      &      & 6082.3901 &       & -2.032 \\
      &      & 6082.3921 &       & -2.077 \\
      &      & 6082.3965 &       & -1.672 \\
 Co I &      & 6082.4214 & 3.514 & -1.989 \\
      &      & 6082.4219 &       & -2.292 \\
      &      & 6082.4263 &       & -1.513 \\
      &      & 6082.4561 &       & -2.000 \\
      &      & 6082.4609 &       & -1.365 \\
      &      & 6082.4956 &       & -2.077 \\
      &      & 6082.5020 &       & -1.229 \\
      &      & 6082.5410 &       & -2.292 \\
      &      & 6093.0952 &       & -3.457 \\
      &      & 6093.1157 &       & -3.046 \\
      &      & 6093.1240 &       & -3.343 \\
      &      & 6093.1392 &       & -3.662 \\
 Co I &      & 6093.1484 & 1.740 & -3.468 \\
      &      & 6093.1597 &       & -3.457 \\
      &      & 6093.1738 &       & -3.644 \\
      &      & 6093.1738 &       & -3.343 \\
      &      & 6093.1846 &       & -3.468 \\
 Co I &      & 6188.9248 & 1.710 & -3.805 \\
      &      & 6188.9370 &       & -3.106 \\
      &      & 6188.9678 &       & -3.624 \\
      &      & 6188.9790 &       & -3.398 \\
      &      & 6188.9912 &       & -3.805 \\
      &      & 6189.0029 &       & -3.593 \\
      &      & 6189.0122 &       & -3.804 \\
      &      & 6189.0239 &       & -3.624 \\
      &      & 6189.0298 &       & -3.657 \\
      &      & 6189.0381 &       & -4.521 \\
      &      & 6189.0479 &       & -3.593 \\
      &      & 6189.0518 &       & -3.856 \\
      &      & 6189.0571 &       & -5.764 \\
      &      & 6189.0649 &       & -3.657 \\
      &      & 6189.0688 &       & -4.111 \\
      &      & 6189.0752 &       & -3.856 \\
      &      & 6454.9331 &       & -1.793 \\
      &      & 6454.9341 &       & -2.056 \\
      &      & 6454.9370 &       & -1.589 \\
      &      & 6454.9438 &       & -1.989 \\
 Co I &      & 6454.9458 & 3.632 & -1.419 \\
      &      & 6454.9541 &       & -1.793 \\
      &      & 6454.9590 &       & -1.273 \\
      &      & 6454.9648 &       & -2.688 \\
      &      & 6454.9678 &       & -1.688 \\
      &      & 6454.9780 &       & -1.144 \\
      &      & 6454.9849 &       & -2.533 \\
      &      & 6454.9868 &       & -1.641 \\
      &      & 6455.0020 &       & -1.028 \\
      &      & 6455.0098 &       & -2.533 \\
      &      & 6455.0122 &       & -1.647 \\
      &      & 6455.0298 &       & -0.923 \\
      &      & 6455.0400 &       & -2.630 \\
      &      & 6455.0410 &       & -1.720 \\
      &      & 6455.0742 &       & -2.834 \\
      &      & 6455.0752 &       & -1.931 \\
      &      & 6455.1138 &       & -3.232 \\
      &      & 6814.8887 &       & -2.839 \\
      &      & 6814.9150 &       & -2.725 \\
      &      & 6814.9238 &       & -2.428 \\
      &      & 6814.9360 &       & -2.850 \\
      &      & 6814.9434 &       & -3.044 \\
 Co I &      & 6814.9688 & 1.956 & -3.026 \\
      &      & 6814.9780 &       & -2.839 \\
      &      & 6814.9873 &       & -2.725 \\
      &      & 6814.9907 &       & -2.850 \\
      &      & 7417.3076 &       & -2.637 \\
      &      & 7417.3491 &       & -2.853 \\
      &      & 7417.3838 &       & -3.136 \\
 Co I &      & 7417.3853 & 2.042 & -3.263 \\
      &      & 7417.4126 &       & -3.102 \\
      &      & 7417.4141 &       & -3.575 \\
      &      & 7417.4355 &       & -3.110 \\
      &      & 7417.4487 &       & -4.128 \\
      &      & 7417.4517 &       & -3.274 \\
      &      & 7417.4639 &       & -3.700 \\
      &      & 7417.4736 &       & -3.450 \\
      &      & 7417.4766 &       & -3.274 \\
 Ni I & 1353 & 5748.3599 & 1.680 & -3.240 \\
      &      & 5749.2793 &       & -2.526 \\
 Ni I &      & 5749.3037 & 3.941 & -2.112 \\
 Ni I &      & 5754.6699 & 1.930 & -1.850 \\
 Ni I &      & 5805.2202 & 4.168 & -0.620 \\
 Ni I &      & 5847.0098 & 1.676 & -3.410 \\
 Ni I &      & 5996.7402 & 4.236 & -1.010 \\
 Ni I &      & 6007.3169 & 1.677 & -3.410 \\
 Ni I &      & 6086.2881 & 4.266 & -0.460 \\
 Ni I &      & 6108.1201 & 1.680 & -2.430 \\
 Ni I &      & 6111.0801 & 4.088 & -0.810 \\
 Ni I &      & 6119.7598 & 4.270 & -1.316 \\
 Ni I &      & 6128.9839 & 1.677 & -3.360 \\
 Ni I &      & 6130.1401 & 4.266 & -0.940 \\
 Ni I &      & 6133.9800 & 4.090 & -1.910 \\
 Ni I &      & 6175.3701 & 4.089 & -0.550 \\
 Ni I &      & 6176.7979 & 4.088 & -0.260 \\
 Ni I &      & 6177.2500 & 1.826 & -3.510 \\
 Ni I &      & 6186.7168 & 4.106 & -0.880 \\
 Ni I &      & 6204.6050 & 4.088 & -1.100 \\
      &      & 6223.9712 &       & -1.466 \\
 Ni I &      & 6223.9912 & 4.105 & -1.052 \\
 Ni I &      & 6230.1001 & 4.110 & -1.132 \\
 Ni I &      & 6322.1689 & 4.154 & -1.210 \\
 Ni I &      & 6327.6001 & 1.680 & -3.060 \\
      &      & 6378.2329 &       & -1.386 \\
 Ni I &      & 6378.2578 & 4.154 & -0.972 \\
 Ni I &      & 6482.8101 & 1.930 & -2.760 \\
 Ni I &      & 6598.6108 & 4.236 & -0.910 \\
 Ni I &      & 6635.1299 & 4.420 & -0.720 \\
 Ni I &      & 6643.6401 & 1.676 & -2.030 \\
 Ni I &      & 6767.7798 & 1.830 & -2.100 \\
 Ni I &      & 6772.3198 & 3.658 & -0.970 \\
 Ni I &      & 6842.0430 & 3.658 & -1.500 \\
 Ni I &      & 7110.8999 & 1.940 & -2.880 \\
 Ni I &      & 7715.5908 & 3.700 & -1.010 \\
 Ni I &      & 7748.8901 & 3.700 & -0.380 \\
 Ni I &      & 7788.9302 & 1.950 & -1.750 \\
 Ni I &      & 7826.7700 & 3.700 & -1.840 \\
      &      & 7933.0918 &       & -1.383 \\
      &      & 7933.1011 &       & -1.035 \\
      &      & 7933.1152 &       & -1.383 \\
      &      & 7933.1221 &       & -1.035 \\
 Cu I &      & 7933.1309 & 3.790 & -2.082 \\
      &      & 7933.1362 &       & -1.734 \\
      &      & 7933.1538 &       & -1.383 \\
      &      & 7933.1572 &       & -1.035 \\
      &      & 8092.6001 &       & -2.055 \\
      &      & 8092.6079 &       & -1.707 \\
      &      & 8092.6079 &       & -1.356 \\
      &      & 8092.6172 &       & -1.008 \\
      &      & 8092.6230 &       & -0.909 \\
 Cu I &      & 8092.6289 & 3.817 & -0.561 \\
      &      & 8092.6362 &       & -1.754 \\
      &      & 8092.6396 &       & -1.406 \\
      &      & 8092.6396 &       & -1.356 \\
      &      & 8092.6440 &       & -1.008 \\
      &      & 8092.6489 &       & -1.356 \\
      &      & 8092.6538 &       & -1.008 \\
 Zn I &  726 & 6362.3472 & 5.800 &  0.140 \\
Ba II & 1455 & 5853.6958 & 0.604 & -2.915 \\
      &      & 5853.6968 &       & -2.857 \\
      &      & 5853.6968 &       & -3.148 \\
      &      & 5853.6982 &       & -3.090 \\
      &      & 5853.6992 &       & -3.295 \\
      &      & 5853.6992 &       & -3.061 \\
      &      & 5853.7002 &       & -2.760 \\
      &      & 5853.7002 &       & -3.693 \\
      &      & 5853.7002 &       & -2.546 \\
      &      & 5853.7002 &       & -2.530 \\
      &      & 5853.7002 &       & -3.459 \\
      &      & 5853.7002 &       & -2.313 \\
      &      & 5853.7002 &       & -1.054 \\
      &      & 5853.7002 &       & -2.012 \\
      &      & 5853.7002 &       & -2.994 \\
      &      & 5853.7012 &       & -3.295 \\
      &      & 5853.7021 &       & -3.061 \\
      &      & 5853.7031 &       & -2.857 \\
      &      & 5853.7031 &       & -3.090 \\
      &      & 5853.7041 &       & -3.148 \\
      &      & 5853.7041 &       & -2.915 \\
Ba II &      & 6141.6948 & 0.704 & -3.641 \\
      &      & 6141.6948 &       & -3.407 \\
      &      & 6141.6968 &       & -2.495 \\
      &      & 6141.6968 &       & -2.261 \\
      &      & 6141.6982 &       & -3.465 \\
      &      & 6141.6982 &       & -3.231 \\
      &      & 6141.6992 &       & -1.686 \\
      &      & 6141.6992 &       & -1.453 \\
      &      & 6141.6992 &       & -2.398 \\
      &      & 6141.6992 &       & -2.164 \\
      &      & 6141.7002 &       & -1.700 \\
      &      & 6141.7002 &       & -0.224 \\
      &      & 6141.7002 &       & -1.182 \\
      &      & 6141.7012 &       & -1.892 \\
      &      & 6141.7012 &       & -1.659 \\
      &      & 6141.7012 &       & -2.510 \\
      &      & 6141.7012 &       & -2.277 \\
      &      & 6141.7021 &       & -1.909 \\
      &      & 6141.7021 &       & -2.465 \\
      &      & 6141.7021 &       & -2.143 \\
      &      & 6141.7031 &       & -2.231 \\
      &      & 6496.8882 &       & -2.832 \\
      &      & 6496.8892 &       & -3.066 \\
      &      & 6496.8911 &       & -2.133 \\
      &      & 6496.8921 &       & -2.367 \\
      &      & 6496.8960 &       & -1.919 \\
      &      & 6496.8960 &       & -1.686 \\
Ba II &      & 6496.8999 & 0.604 & -2.000 \\
      &      & 6496.8999 &       & -1.482 \\
      &      & 6496.8999 &       & -0.524 \\
      &      & 6496.9058 &       & -2.764 \\
      &      & 6496.9058 &       & -2.531 \\
      &      & 6496.9072 &       & -2.367 \\
      &      & 6496.9082 &       & -2.133 \\
      &      & 6496.9102 &       & -2.367 \\
      &      & 6496.9121 &       & -2.133 \\


==> pars.tex <==
\\ \multicolumn{11}{c}{wm: late F dwarfs} \\ \hline
   522 & 6281 & 4.252 &  0.113 & 1.48 &  131 & 25 &  0.102 & 0.029 & -0.087 & 0.012 \\
  3119 & 6246 & 4.374 &  0.127 & 1.30 &   96 & 18 &  0.224 & 0.032 & -0.073 & 0.011 \\
  3236 & 6309 & 4.399 &  0.097 & 1.25 &  159 & 25 &  0.249 & 0.036 & -0.103 & 0.014 \\
  3540 & 6104 & 4.186 &  0.002 & 1.12 &  -46 & 16 &  0.036 & 0.032 & -0.198 & 0.015 \\
  5862 & 6111 & 4.359 &  0.173 & 1.18 &  -39 & 12 &  0.209 & 0.032 & -0.027 & 0.012 \\
  5985 & 6106 & 4.414 &  0.084 & 1.19 &  -44 & 11 &  0.264 & 0.029 & -0.116 & 0.010 \\
  7978 & 6114 & 4.412 & -0.023 & 1.13 &  -36 & 11 &  0.262 & 0.036 & -0.223 & 0.014 \\
  8548 & 6043 & 4.277 &  0.016 & 1.22 & -107 & 11 &  0.127 & 0.029 & -0.184 & 0.012 \\
 12653 & 6147 & 4.419 &  0.156 & 1.16 &   -3 & 11 &  0.269 & 0.029 & -0.044 & 0.010 \\
 12764 & 6211 & 4.349 &  0.082 & 1.28 &   61 & 12 &  0.199 & 0.025 & -0.118 & 0.009 \\
 14194 & 6387 & 4.384 &  0.186 & 1.33 &  237 & 28 &  0.234 & 0.032 & -0.014 & 0.011 \\
 14857 & 6143 & 4.270 &  0.126 & 1.28 &   -7 & 12 &  0.120 & 0.025 & -0.074 & 0.011 \\
 14954 & 6150 & 4.150 &  0.200 & 1.40 &    0 &  0 &  0.000 & 0.000 &  0.000 & 0.000 \\
 17819 & 6119 & 4.180 &  0.146 & 1.24 &  -31 & 13 &  0.030 & 0.025 & -0.054 & 0.012 \\
 22919 & 6075 & 4.363 &  0.050 & 1.10 &  -75 & 11 &  0.213 & 0.032 & -0.150 & 0.012 \\
 25388 & 6065 & 4.249 &  0.013 & 1.27 &  -85 & 10 &  0.099 & 0.025 & -0.187 & 0.011 \\
 27075 & 6011 & 4.361 &  0.007 & 1.09 & -139 & 10 &  0.211 & 0.032 & -0.193 & 0.013 \\
 28913 & 6218 & 4.218 &  0.170 & 1.34 &   68 & 17 &  0.068 & 0.025 & -0.030 & 0.011 \\
 30711 & 6146 & 4.235 &  0.010 & 1.35 &   -4 & 11 &  0.085 & 0.032 & -0.190 & 0.013 \\
 37645 & 6137 & 4.164 &  0.052 & 1.42 &  -13 & 15 &  0.014 & 0.029 & -0.148 & 0.013 \\
 41134 & 5988 & 4.408 &  0.086 & 1.05 & -162 &  9 &  0.258 & 0.032 & -0.114 & 0.012 \\
 41226 & 6273 & 4.335 &  0.186 & 1.30 &  123 & 23 &  0.185 & 0.036 & -0.014 & 0.014 \\
 41968 & 6152 & 4.304 &  0.016 & 1.30 &    2 & 11 &  0.154 & 0.029 & -0.184 & 0.011 \\
 42123 & 6008 & 4.133 &  0.054 & 1.23 & -142 & 10 & -0.017 & 0.021 & -0.146 & 0.011 \\
 42723 & 6015 & 4.219 &  0.088 & 1.20 & -135 & 11 &  0.069 & 0.029 & -0.112 & 0.012 \\
 48351 & 6037 & 4.070 &  0.084 & 1.35 & -113 & 12 & -0.080 & 0.025 & -0.116 & 0.012 \\
 48376 & 6163 & 4.349 &  0.063 & 1.20 &   13 & 12 &  0.199 & 0.029 & -0.137 & 0.011 \\
 53196 & 6089 & 4.337 &  0.108 & 1.21 &  -61 & 11 &  0.187 & 0.029 & -0.092 & 0.012 \\
 54383 & 6137 & 4.278 &  0.085 & 1.27 &  -13 & 10 &  0.128 & 0.029 & -0.115 & 0.011 \\
 60353 & 6164 & 4.380 &  0.166 & 1.20 &   14 & 12 &  0.230 & 0.036 & -0.034 & 0.013 \\
 67408 & 6105 & 4.402 & -0.002 & 1.17 &  -45 & 12 &  0.252 & 0.032 & -0.202 & 0.011 \\
 70782 & 6170 & 4.347 &  0.132 & 1.22 &   20 &  9 &  0.197 & 0.029 & -0.068 & 0.010 \\
 73754 & 6072 & 4.468 &  0.006 & 1.18 &  -78 & 12 &  0.318 & 0.036 & -0.194 & 0.014 \\
 79346 & 5985 & 4.410 &  0.108 & 1.03 & -165 & 10 &  0.260 & 0.032 & -0.092 & 0.013 \\
 81062 & 6285 & 4.287 &  0.151 & 1.34 &  135 & 25 &  0.137 & 0.032 & -0.049 & 0.011 \\
 83547 & 6016 & 4.255 & -0.014 & 1.17 & -134 &  9 &  0.105 & 0.029 & -0.214 & 0.012 \\
 84827 & 6080 & 4.197 &  0.166 & 1.09 &  -70 &  9 &  0.047 & 0.025 & -0.034 & 0.011 \\
 84856 & 6055 & 3.986 &  0.166 & 1.36 &  -95 & 14 & -0.164 & 0.032 & -0.034 & 0.013 \\
 90485 & 6258 & 4.071 &  0.106 & 1.50 &  108 & 26 & -0.079 & 0.029 & -0.094 & 0.014 \\
 92233 & 5966 & 4.011 &  0.026 & 1.31 & -184 &  8 & -0.139 & 0.025 & -0.174 & 0.011 \\
 94645 & 6230 & 4.440 &  0.196 & 1.22 &   80 & 17 &  0.290 & 0.032 & -0.004 & 0.012 \\
 95164 & 6047 & 4.186 &  0.017 & 1.30 & -103 & 12 &  0.036 & 0.029 & -0.183 & 0.013 \\
 96078 & 6111 & 4.253 & -0.030 & 1.27 &  -39 & 12 &  0.103 & 0.039 & -0.230 & 0.016 \\
 97546 & 6089 & 4.296 &  0.096 & 1.21 &  -61 & 12 &  0.146 & 0.025 & -0.104 & 0.011 \\
 97675 & 6124 & 4.213 &  0.130 & 1.29 &  -26 & 14 &  0.063 & 0.029 & -0.070 & 0.013 \\
100072 & 6140 & 4.444 &  0.056 & 1.13 &  -10 & 13 &  0.294 & 0.032 & -0.144 & 0.013 \\
100396 & 6160 & 4.153 &  0.075 & 1.44 &   10 & 17 &  0.003 & 0.029 & -0.125 & 0.013 \\
104071 & 6008 & 4.335 &  0.098 & 1.15 & -142 & 10 &  0.185 & 0.032 & -0.102 & 0.013 \\
108859 & 6059 & 4.445 &  0.003 & 1.17 &  -91 & 11 &  0.295 & 0.032 & -0.197 & 0.013 \\
113086 & 6183 & 4.309 &  0.035 & 1.27 &   33 & 14 &  0.159 & 0.029 & -0.165 & 0.011 \\
114096 & 6151 & 4.348 &  0.102 & 1.25 &    1 & 13 &  0.198 & 0.032 & -0.098 & 0.011 \\
114670 & 6151 & 4.350 &  0.131 & 1.18 &    1 & 12 &  0.200 & 0.029 & -0.069 & 0.010 \\
\\ \multicolumn{11}{c}{mr: metal-rich solar analogs} \\ \hline
  1499 & 5729 & 4.365 &  0.139 & 1.06 &  -21 &  9 &  0.065 & 0.024 & -0.111 & 0.013 \\
  1803 & 5837 & 4.516 &  0.178 & 1.31 &   87 & 16 &  0.216 & 0.024 & -0.072 & 0.016 \\
  5176 & 5864 & 4.385 &  0.135 & 1.10 &  114 & 16 &  0.085 & 0.024 & -0.115 & 0.012 \\
 12048 & 5769 & 4.164 &  0.105 & 1.17 &   19 & 14 & -0.136 & 0.024 & -0.145 & 0.016 \\
 12186 & 5817 & 4.146 &  0.096 & 1.22 &   67 & 15 & -0.154 & 0.024 & -0.154 & 0.015 \\
 17054 & 5826 & 4.249 &  0.346 & 1.24 &   76 & 10 & -0.051 & 0.017 &  0.096 & 0.010 \\
 17960 & 5804 & 4.267 &  0.159 & 1.14 &   54 & 11 & -0.033 & 0.020 & -0.091 & 0.012 \\
 20723 & 5638 & 4.356 &  0.196 & 0.96 & -112 &  9 &  0.056 & 0.020 & -0.054 & 0.011 \\
 20741 & 5826 & 4.519 &  0.145 & 1.19 &   76 & 16 &  0.219 & 0.024 & -0.105 & 0.017 \\
 21923 & 5784 & 4.197 &  0.220 & 1.17 &   34 & 11 & -0.103 & 0.017 & -0.030 & 0.012 \\
 22336 & 5928 & 4.186 &  0.216 & 1.27 &  178 & 21 & -0.114 & 0.020 & -0.034 & 0.013 \\
 24681 & 5830 & 4.226 &  0.087 & 1.17 &   80 & 16 & -0.074 & 0.024 & -0.163 & 0.015 \\
 26935 & 5827 & 4.252 &  0.156 & 1.16 &   77 & 15 & -0.048 & 0.020 & -0.094 & 0.013 \\
 29349 & 5912 & 4.233 &  0.227 & 1.27 &  162 & 18 & -0.067 & 0.017 & -0.023 & 0.012 \\
 30243 & 5808 & 4.337 &  0.265 & 1.10 &   58 & 13 &  0.037 & 0.020 &  0.015 & 0.012 \\
 30480 & 5882 & 4.249 &  0.175 & 1.19 &  132 & 17 & -0.051 & 0.024 & -0.075 & 0.014 \\
 31540 & 5676 & 4.362 &  0.216 & 1.01 &  -74 &  8 &  0.062 & 0.014 & -0.034 & 0.009 \\
 34879 & 5906 & 4.391 &  0.263 & 1.12 &  156 & 16 &  0.091 & 0.027 &  0.013 & 0.014 \\
 37309 & 5815 & 4.351 &  0.262 & 1.09 &   65 & 13 &  0.051 & 0.020 &  0.012 & 0.011 \\
 39417 & 5710 & 4.353 &  0.261 & 1.03 &  -40 &  6 &  0.053 & 0.014 &  0.011 & 0.007 \\
 40761 & 5842 & 4.320 &  0.239 & 1.14 &   92 & 12 &  0.020 & 0.020 & -0.011 & 0.011 \\
 40952 & 5676 & 4.385 &  0.150 & 0.97 &  -74 & 10 &  0.085 & 0.020 & -0.100 & 0.011 \\
 51579 & 5912 & 4.336 &  0.189 & 1.20 &  162 & 17 &  0.036 & 0.024 & -0.061 & 0.013 \\
 52409 & 5745 & 4.376 &  0.261 & 1.02 &   -5 &  9 &  0.076 & 0.020 &  0.011 & 0.011 \\
 57291 & 5671 & 4.299 &  0.288 & 1.01 &  -79 &  8 & -0.001 & 0.014 &  0.038 & 0.009 \\
 60081 & 5760 & 4.343 &  0.269 & 1.03 &   10 & 11 &  0.043 & 0.020 &  0.019 & 0.011 \\
 60370 & 5880 & 4.459 &  0.142 & 1.11 &  130 & 16 &  0.159 & 0.027 & -0.108 & 0.016 \\
 61379 & 5841 & 4.107 &  0.275 & 1.27 &   91 & 12 & -0.193 & 0.017 &  0.025 & 0.012 \\
 61595 & 5868 & 4.317 &  0.216 & 1.15 &  118 & 13 &  0.017 & 0.024 & -0.034 & 0.013 \\
 62345 & 5761 & 4.296 &  0.232 & 1.09 &   11 &  8 & -0.004 & 0.014 & -0.018 & 0.008 \\
 65808 & 5664 & 4.329 &  0.204 & 1.02 &  -86 &  8 &  0.029 & 0.017 & -0.046 & 0.011 \\
 70123 & 5894 & 4.426 &  0.219 & 1.09 &  144 & 14 &  0.126 & 0.024 & -0.031 & 0.014 \\
 71803 & 5814 & 4.416 &  0.217 & 1.06 &   64 &  9 &  0.116 & 0.017 & -0.033 & 0.008 \\
 73408 & 5864 & 4.394 &  0.281 & 1.12 &  114 & 16 &  0.094 & 0.024 &  0.031 & 0.012 \\
 74500 & 5750 & 4.300 &  0.250 & 1.10 &    0 &  0 &  0.000 & 0.000 &  0.000 & 0.000 \\
 77740 & 5890 & 4.478 &  0.093 & 1.10 &  140 & 14 &  0.178 & 0.020 & -0.157 & 0.012 \\
 78955 & 5875 & 4.297 &  0.290 & 1.18 &  125 & 14 & -0.003 & 0.024 &  0.040 & 0.014 \\
 81022 & 5928 & 4.194 &  0.263 & 1.30 &  178 & 22 & -0.106 & 0.024 &  0.013 & 0.014 \\
 81767 & 5808 & 4.291 &  0.261 & 1.15 &   58 &  8 & -0.009 & 0.017 &  0.011 & 0.010 \\
 83906 & 5790 & 4.120 &  0.273 & 1.25 &   40 &  8 & -0.180 & 0.010 &  0.023 & 0.009 \\
 86796 & 5770 & 4.244 &  0.263 & 1.13 &   20 &  8 & -0.056 & 0.014 &  0.013 & 0.010 \\
 90593 & 5797 & 4.266 &  0.274 & 1.12 &   47 &  9 & -0.034 & 0.017 &  0.024 & 0.010 \\
 91332 & 5734 & 4.157 &  0.175 & 1.10 &  -16 & 14 & -0.143 & 0.020 & -0.075 & 0.015 \\
 94256 & 5699 & 4.084 &  0.223 & 1.18 &  -51 & 10 & -0.216 & 0.017 & -0.027 & 0.012 \\
 95740 & 5936 & 4.372 &  0.267 & 1.15 &  186 & 14 &  0.072 & 0.024 &  0.017 & 0.013 \\
 98589 & 5862 & 4.486 &  0.178 & 1.10 &  112 & 14 &  0.186 & 0.020 & -0.072 & 0.014 \\
 99115 & 5638 & 4.195 &  0.213 & 1.10 & -112 &  9 & -0.105 & 0.014 & -0.037 & 0.010 \\
 99727 & 5791 & 4.248 &  0.196 & 1.17 &   41 & 11 & -0.052 & 0.017 & -0.054 & 0.011 \\
 99729 & 5711 & 4.108 &  0.185 & 1.20 &  -39 &  9 & -0.192 & 0.014 & -0.065 & 0.011 \\
100500 & 5666 & 4.061 &  0.158 & 1.17 &  -84 &  7 & -0.239 & 0.014 & -0.092 & 0.010 \\
101806 & 5906 & 4.310 &  0.205 & 1.24 &  156 & 19 &  0.010 & 0.024 & -0.045 & 0.013 \\
103682 & 5955 & 4.351 &  0.234 & 1.23 &  205 & 17 &  0.051 & 0.024 & -0.016 & 0.012 \\
106006 & 5755 & 4.396 &  0.148 & 1.05 &    5 & 10 &  0.096 & 0.020 & -0.102 & 0.010 \\
109355 & 5730 & 4.381 &  0.225 & 1.02 &  -20 &  9 &  0.081 & 0.020 & -0.025 & 0.010 \\
110161 & 5952 & 4.314 &  0.246 & 1.23 &  202 & 16 &  0.014 & 0.027 & -0.004 & 0.013 \\
110843 & 5664 & 4.311 &  0.255 & 1.01 &  -86 &  8 &  0.011 & 0.017 &  0.005 & 0.010 \\
113137 & 5853 & 4.221 &  0.205 & 1.20 &  103 & 13 & -0.079 & 0.017 & -0.045 & 0.011 \\
115100 & 5866 & 4.174 &  0.154 & 1.21 &  116 & 18 & -0.126 & 0.024 & -0.096 & 0.015 \\
116852 & 5829 & 4.225 &  0.150 & 1.21 &   79 & 13 & -0.075 & 0.020 & -0.100 & 0.013 \\

